Boosting Cloud Data Analytics using Multi-Objective Optimization

Data analytics in the cloud has become an integral part of enterprise businesses. Big data analytics systems, however, still lack the ability to take user performance goals and budgetary constraints for a task, collectively referred to as task objectives, and automatically configure an analytic job to achieve these objectives. This paper presents a data analytics optimizer that can automatically determine a cluster configuration with a suitable number of cores as well as other system parameters that best meet the task objectives. At a core of our work is a principled multi-objective optimization (MOO) approach that computes a Pareto optimal set of job configurations to reveal tradeoffs between different user objectives, recommends a new job configuration that best explores such tradeoffs, and employs novel optimizations to enable such recommendations within a few seconds. We present efficient incremental algorithms based on the notion of a Progressive Frontier for realizing our MOO approach and implement them into a Spark-based prototype. Detailed experiments using benchmark workloads show that our MOO techniques provide a 2-50x speedup over existing MOO methods, while offering good coverage of the Pareto frontier. When compared to Ottertune, a state-of-the-art performance tuning system, our approach recommends configurations that yield 26\%-49\% reduction of running time of the TPCx-BB benchmark while adapting to different application preferences on multiple objectives.

==> modeling.tex <==
\section{Learning Performance Models}
\label{sec:modelling}

Accurate models for user objectives  are of vital importance because the multi-objective optimizer relies  on such models for computing the Pareto frontier and choosing a better job configuration. 
As stated before, the frequent use of machine learning and UDFs in data analytics today leads to a blackbox approach to modeling in our work. 
In addition, to adapt to diverse user objectives and  complex runtime behaviors 
%involving CPU, IO, shuffling, stragglers, etc., 
we propose to replace static modeling with {\em in-situation modeling}, which learns a model for each user objective in the same computing environment as the user job is executed. 

Our solution to the modeling problem embodies the following ideas. 
First, we explore Deep Learning for in-situation modeling due to its flexibility to learn non-linear models, hence eliminating any modeling assumptions that may fail in practice, and its known strength for representation learning, which allows us to extract meaningful characteristics from runtime metrics of a dataflow program given as a blackbox. 
Second, we aim to train a model of each objective  using all past jobs so that ($i$) these jobs reflect characteristics of the computing environment and ($ii$)  a new job can be mapped to a similar  job in the past to boost the prediction accuracy for the new job,  eliminating the need to explore a large number of configurations for modeling the new job.

%LONGER VERSION
%Furthermore, we explore Deep Learning for in-situation modeling due to its flexibility to learn non-linear models, hence eliminating any modeling assumptions that may fail in practice.
%We also show that such NN based architectures allow us to have compact representations of the workload encodings that preserve similarities across the workloads. Such compact representations are crucial for workload mapping, because attempting to calculate distances using full trace vectors is object to the curse of dimensionality.
%In addition, we train a model using all past workloads so that the new job can be mapped well to a past job to boost the accuracy of prediction of the new job. Even if the jobs are not similar, we can still learn the  the environment from past jobs and adapt to new workloads without having to do a lot of exploration for new jobs. 
% Deep Learning models allows us indeed to learn the environment from past jobs and adapt to new workloads without having to do a lot of exploration for new jobs in contrast to other invasive approaches that waste computation cost during their exploration phase. 


%OLD TEXT
%Moreover, since today's analytic tasks can be encoded in any popular programming language, modeling tools must be able to handle programs given as black boxes. In addition, static, hard-coded models~\cite{HerodotouB11,Jalaparti+12:model,LiDS15,RajanKCK16}  %Ferguson+12:model
%often fail to adapt to new user performance objectives, new workloads, new versions of the software system, new hardware, etc. 
%For all of the above reasons, we argue for a new approach called {\em in-situation modeling}, that is, learning a model for each user objective in the same computing environment as the user job is being executed. 

%KHALED'S TEXT
%Having accurate objective models is of extreme importance because the multi-objective optimizer, as we've seen in the last section, relies heavily on such models. Traditional cost models used with RDBMS are not a good option for more recent Big Data systems because such systems extend the support of the well known algebra operators to incorporate other arbitrary operators and user defined functions coded in Java or Scala for example. Therefore, instead of using analytical and hard coded models with such complex systems, we have to leverage statistical models built using machine learning. We show in this section that it's possible to build models for different objectives using machine learning algorithms that leverage data collected from workload runs and achieve low error predictions. We start by introducing the notation used for modeling, and then we delve gradually into more formalism, and then we end this section with an extensive description of our proposed architectures for modeling.

%Notation
%Challenges even for DL: lack of workload encodings

\subsection{Formalism and Challenges}

When a user submits a job, she specifies a set of objectives, %optionally with constraints on these objectives,  
and an initial job configuration. During execution, job $j$ produces a trace, $T_j^i (\theta_j^i, O_j^i)$, that corresponds to the current ($i^{th}$) configuration, $\theta_j^i$, and includes the {\em observation vector}, $O_j^i$. Recall from Section~\ref{sec:problem} that the observation vector  contains 
objective-related,  
application-level, %like the number of bytes written/read  by Spark, 
and OS metrics. %regarding the CPU, memory, and I/O. 
We use $T_j$ to denote the traces obtained with all configurations for job $j$, and $T$ to denote all available traces. 

The goal of modeling is to build a predictive model for each user objective using $T$, and later use the model to  predict  the performance of this objective for a new job $j'$ and a particular configuration $\theta_{j'}$. Learning such models is challenging because a model depends  not only on the configuration but also on the workload characteristics of each job. When the dataflow program for the job is treated as a blackbox, the workload characteristics are missing both from the training data, $T$, for building the model, and from the trace of a new job, over which the optimizer requests the model to predict the performance under a given configuration. 

Therefore, the modeling task is complicated by the need to extract the {\em workload  encoding}, $W_j$, from the traces for job $j$. In our system,  $W_j$ is a numerical vector that contains useful information about the dataflow program on a given dataset, e.g., CPU cycles or memory footprint per tuple processed by the program, and other factors that may not be known in advance. $W_j$ has to be inferred automatically from traces of job $j$. 
%$(T_j^1, ..., T_j^{i}, ...)$ obtained with configurations $(\theta_j^1, .., \theta_j^{i}, ...)$. 
We give a more formal definition of the workload encoding as follows.

\begin{definition}
	{\bf The Workload Encoding $W_j$} %(for ease of notation, we drop the $j$ index whenever no confusion)
	is a compact real-valued vector that encodes the characteristics of a specific dataflow program (also called job or workload) on a given dataset,  and satisfies three conditions:
	\skipzerolist
		\item {\bf 1) Invariance}. For the same logical dataflow program and the same dataset,  $W_j$ should be (approximately) an invariant in order to represent the workload.
		\item {\bf 2) Reconstruction}. $W_j$ should carry all the information for reconstructing the observation $O_j^i$, given $\theta_j^i$.
		\item {\bf 3) Similarity-preserving}. If two workloads $j$ and $j'$ are similar in the sense that given each configuration, their observation vectors are similar (under a vector-based distance function), their encodings $W_j$ and $W_j'$ should also be similar in the encoding space.
%		$W_j$ should preserve similarities among workloads {\color{red} under the same datasets?}. If two workloads $j$ and $j'$, considered as blackboxes, are close enough, the distance between their encodings $W_j$ and $W_j'$ should be small.
	\end{list}
\end{definition}
\noindent Obviously, we wish to have the encoding much smaller than the observation vector in order to avoid many learning problems due to the ``curse of dimensionality''.

%\textbf{Formal description of the modeling system}
Given the notion of workload encodings, we next define the learning problem. 
Without loss of generality, let us consider latency $l$ as a user objective. 
The model  for latency can be formulated as a deterministic function $\Psi$ s.t.
$$
	\Psi(\theta_j^i, W_j) = l_j^i
$$
\noindent The learning problem is to choose the function that  minimizes the distance between the predicted latency and the actual latency for all (job, configuration) combinations, called {\em training instances}, in the training data:
$$
\Psi^*=\underset{\Psi}{\text{arg min}} \hspace{0.3cm} \text{avg}\big( \text{distance}\big(\Psi(\theta_j^i, W_j), l_j^i \big) \big)
$$
where the average is taken among all the training instances.
If both $\theta_j^i$ and $W_j$ were given, the problem would be a classic learning problem. Since $W_j$ is unknown, we need to extend  existing learning tools to extract $W_j$. In the following, we propose two neural network architectures that simultaneously extract the workload encoding from a job and build a predictive model on the configuration and  encoding. 
%the embedding and the autoencoder architectures.

\begin{figure*}[t]
\centering
\vspace{-0.1in}
\begin{tabular}{cc}

\hspace{-0.1in}
\subfigure[\small{Embedding  architecture}]
{\label{fig:embedding-architecure}\includegraphics[width=5.83cm,height=3.8cm]{figures2/embedding.pdf}}
%figures/embedding-architecture

&
\hspace{0.2in}
\subfigure[\small{Auto-encoder architecture}]
{\label{fig:auto-encoder}\includegraphics[width=8.81cm,height=3.8cm]{figures2/autoencoder.pdf}}
%figures/autoencoder-architecture

\end{tabular}
\vspace{-0.2in}
\caption{\small Two neural network architectures for extracting the workload encoding and learning a predictive model. }\label{fig:models}
\vspace{-0.1in}
\end{figure*}

%\begin{figure}[H]
%\begin{center}
%\includegraphics[scale=.35]{figures/embeddings}
%\end{center}
%\caption{Embedding Deep Learning Architecture}
%\label{fig: embedding-architecure}
%\end{figure}
%
%\begin{figure}[H]
%         \begin{center}
%          \includegraphics[scale=.5]{figures/auto-encoder}
%          \caption{An Auto-Encoder Deep Learning Architecture with depth=2}
%          \label{fig: auto-encoder}
%         \end{center}
%        \end{figure}


%------------------------------------------------------------------
\subsection{Embedding Approach}
\label{subsec:embedding}

The embedding approach extracts the workload encoding and builds a predictive (regression) model for a user objective   in the same neural network architecture. 
As shown in Figure \ref{fig:embedding-architecure}, the encoding extraction part is coupled with the regression part, and the same training strategy (back propagation) will be used to learn both simultaneously. 
 The idea of embedding comes from %the neural network architectures used in 
deep recommender systems where user profiles are embedded in vectors of values to reflect the user rankings of movies or books~\cite{He:2017:NCF:3038912.3052569}. 
%\cite{He:2017:NCF:3038912.3052569, 45530, 6779506, DBLP:journals/corr/ChenHSS17, Lian:2017:CCC:3041021.3054207}. 
In our context of learning workload encodings, we aim to embed the information on workload characteristics in a vector, whose values are learned in the training process as described below.
%and fill the vector with meaningful values based on the performance achieved by the workload under a configuration.
%\todo{Redraw the plots}
%\begin{figure}[H]
%\begin{center}
%\includegraphics[scale=.35]{figures/embeddings}
%\end{center}
%\caption{Embedding Deep Learning Architecture}
%\label{fig: embedding-architecure}
%\end{figure}

\cut{
\begin{itemize}
  \item Shape of the embedding matrix: $(n \times p)$
  \item Shape of the configuration matrix: $(m \times 4)$
\end{itemize}
with n is the total number of different jobs, p is the dimension of the embedding, and m is the total number of training points.
}
%The input of the neural network architecture is ($j$, $\theta_j^i$) and the output is $f(\theta_j^i)$, where $j$ is the id of the job. 

This neural network architecture consists of three layers:
 (1) An embedding layer with a weight matrix $W$, which includes a row vector $W_j$ for each job $j$. $W_j$ is called the embedding vector or the workload encoding. Each $W_j$ is  initialized  randomly and later adjusted during training. %using backpropagation. 
 (2) A concatenation layer concatenates the embedding vector $W_j$  with an input configuration $\theta_j^i$, denoted as $<W_j, \theta_j^i>$, for job $j$.
  (3) Several fully connected (FC) layers that take $<W_j, \theta_j^i>$ as the  input and produce $h(\theta_j^i)$ as the final output.
$W_j$ contributes implicitly to the output function $h(\theta_j^i) \equiv h(W_j, \theta_j^i)$ because it is learned within the model.
%\textbf{\textit{Note}}: $W_j$ contributes implicitly to $f$: $ f(W_j, \theta_j^i) \equiv f(\theta_j^i)$ but $W_j$ is omitted since it's not provided as input but is learnt.

{\bf Training Strategy}.
The embedding approach requires training every time a new job is submitted. It is because the the embedding vector for the new job is randomly initialized and can only be adjusted by triggering the training process. Nevertheless, we can employ an {\em incremental training} strategy: when the trace of a new job  becomes available, we invoke training using only the new trace. During backpropagation, only the  embedding vector of the current job gets updated to become more meaningful; the weights in the fully connected layers may be updated as well.
%Nevertheless, the architecture allows us to predict with a small overhead after incrementally training on the new job over several epochs. 
%While incrementally training over the new job's trace, the new job's embedding vector gets updated during back-propagation to become more meaningful.

%This architecture allows us to pretrain the embedding layer by using all the observations $O_j^i$ (or $\phi_j^i$ for the scaled version) collected from training samples, and this by simply changing the last layer of the neural network architecture (changing the dimension of the output to be equal to the dimension of $O_j^i$ instead of being a scalar), and changing the loss function to be the mean squared error between the output $f'(\theta_j^i)$ (which is a vector now) and $O_j^i$ instead of being the mean squared error between the output $f(\theta_j^i)$ (a scalar) and $l_j^i$ 

{\bf Limitation}. A major issue with the embedding approach is how to set  the output function $h(\theta_j^i)$. 
To fulfill the reconstruction requirement, $h(\theta_j^i)$ can be treated as the prediction of the observation vector $O_j^i$ with configuration $\theta^i_j$. 
However, the user objective (e.g., latency) is only one number in the large observation vector $O$. A neural network trained to minimize the loss regarding the entire observation vector may incur large error for  latency. Therefore, we restrict the output $h(\theta_j^i)$ to only the latency. Then the embedding approach makes very little use of the full observation vector, and hence 
 is not a winning strategy in our work. In the interest of space, we defer additional details to Appendix~\ref{appendix:modeling}. 

%{\bf Choice of Output Function}. Now we consider the design of the output function $h(\theta_j^i)$. 
%To fulfill the reconstruction requirement stated above, $h(\theta_j^i)$ can be treated an approximation of the observation vector $O_j^i$ with configuration $\theta^i_j$. During the training process, in the backpropagation phase $W$ is adjusted along with the other neural network weights in a way to minimize the loss function:
%      \begin{equation}\label{loss-embedding-pretraining}
%       loss = \displaystyle\frac{1}{m}\displaystyle\sum_{j\in J_{train}}\sum_{i \in I_j}
%        ||h^O(\theta_j^i) - O_j^i||^2
%      \end{equation}
%where $I_j$ refers to the collection of configurations for job $j$, $J_{train}$ is the set of jobs in the training dataset, and $m$ is the total number of training instances, $m = \sum_{j \in J}{|I_j|}$.
%%the number of training points: $m = \displaystyle\sum_{j \in J}{|I_j|}$
%
%However, our goal is to predict a particular target (with latency chosen as an example in the discussion below), which is only one number in the large observation vector $O$. A neural network trained to minimize the loss regarding the entire observation vector may incur large errors for  latency. Therefore, we propose an alternative strategy where the output $h(\theta_j^i)$ includes only the latency, and loss function becomes:
%%Therefore, we propose an alternative strategy where we
%%optimize another loss function $loss'$ that emphasizes on this particular target. Taking latency $l$ as an example, we use $f'(.)$ (which represents now an approximation of the latency, and which is part of the vector $f(.)$) instead of $f(.)$ in the new loss function:
%      \begin{equation}\label{loss-embedding}
%      loss = \displaystyle\frac{1}{m}\displaystyle\sum_{j\in J_{train}}\sum_{i \in I_j}
%      ||h^l(\theta_j^i) - l_j^i||^2
%      \end{equation}
%      
%
%The above discussion reveals several limitations of the embedding approach. 
%First, the training process makes limited use of the full observation trace, as shown in Eq.~\ref{loss-embedding}.
%Second, it requires training, although in an incremental fashion, for each new job  to learn the embedding vector.
%Third, it offers limited sharing of information between different jobs. Only the fully connected layers will leverage training data belonging to different jobs. The embedding vectors, however, are learned independently. Having learned an accurate encoding $W_1$ of the first job does not help much in learning $W_2$ of the second job, even if the two jobs are similar. 






%---------------------------------------------------
\subsection{Autoencoder Approach}
\label{subsec:autoencoder}


The autoencoder approach decouples workload extraction from performance prediction (regression) into two separate architectures, as shown in figure \ref{fig:auto-encoder}. First, it extracts workload encodings using an  autoencoder,  a neural network architecture  for non-linear dimensionality reduction to learn a compact representation of data. In our setting, the autoencoder transforms the observation $O_j$ to a compact encoding $E_j$, the  bottleneck of the architecture. This encoding is learned by trying to reconstruct an approximation $\tilde{O}_j$ of the input  $O_j$, which naturally meets the reconstruction property. 


Then, to model the latency $l_j^i$, we fit a regression function on both the job configuration $\theta_j^i$ and the extracted workload encoding $E_j$. %The function output will be an approximation of the true latency $l_j^i$.
For this, we can use any regression techniques. Our system includes a neural network regressor, a SVM regressor, and a gradient boosting regressor~\cite{hastie01statisticallearning}.




{\bf Invariant encodings.}
While one may think that the intuitive autoencoder architecture that takes the entire encoding $E_j$ as a workload encoding will work properly, it actually violates the invariance property. This is because the input observation $O_j$ is determined by both the variant job configuration, $\theta_j^i$, and the invariant workload encoding, $W_j$. Therefore, the extracted encoding $E_j$ is a mix of both effects. To the best of our knowledge, no existing autoencoder architectures can produce invariant encodings out of variant inputs. Contractive autoencoders \cite{Rifai:2011:CAE:3104482.3104587}, for example, yield localized space contraction, but remain incapable of providing invariant encodings from different inputs. 
To enable invariant workload encodings, we offer several ways to modify both the architecture and the loss function of autoencoders. We describe the best strategy below and leave other options to Appendix~\ref{appendix:modeling}.

%{\em Minimizing variance}.
%One idea is that during training of the autoencoder, we always know the true job configuration in each {\em training instance}. 
%Hence, we can extend the architecture with an intermediate state $\hat{E}_j^i$ at the bottleneck layer to  represent the exact job configuration, which will be used to reconstruct the output 
%$\tilde{O}_j$. Further, we introduce an additional term to the loss function to minimize the variance among  instance level encodings $E_j^i$ that belong to the same job. %(a.k.a. variation coefficient).
%The hope is that $\hat{E}_j^i$ may take care of data reconstruction while minimizing variance among $E_j^i$ may give us  invariant encodings. However, backpropagation fails to achieve our goal and sometimes yields trivial solutions. %where the encodings are not  meaningful. 



{\em Concentrating variance on the job configuration}.
In this architecture, we  force the autoencoder to concentrate the variance of  the encoding $E_j^i$  on the job configuration $\theta_j^i$.
To do so, we break the encoding $E_j^i$ in the bottleneck layer into two parts, as shown in the figure \ref{fig:auto-encoder}. The first  is a variant part $\tilde{E}_j^i$ that  approximates the job configuration $\theta_j^i$, with $|\tilde{E}_j^i| = |\theta_j^i|$. The second part aims to approximate the workload encoding as an invariant $\bar{E}_j^i$. While the size of $\tilde{E}_j^i$ is fixed, the size of $\bar{E}_j^i$  will be determined through hyper-parameter tuning~\cite{Bengio2012}.
To achieve the above goal during backpropagation, we introduce a second term 
%(the term multiplied by the $\gamma$ coefficient) 
to the loss function: 
\begin{equation}\label{loss-ae}
\text{Loss} = \displaystyle\frac{1}{m}\displaystyle\sum_{j\in J_{train}}\sum_{i \in I_j}( ||O_j^i - \tilde{O}_j^i||^2 + \gamma ||\theta_j^i - \tilde{E}_j^i||^2)
\end{equation}
where 
$I_j$ refers to the collection of configurations for job j, 
%and $J_{train}$ represents the set of jobs used in the training setting.
and $\gamma$ is a hyper parameter that controls  how much the approximation of the job configuration contributes to the loss function. By minimizing the loss,  backpropagation may be able to minimize both the data reconstruction error and the approximation error of the job configuration. 

For the remainder of the encoding, $\bar{E}_j^i$, the set of $\bar{E}_j^i$, $i=1,2,...$, are extracted for the same job with different configurations, hence called {\em instance level encodings}.
Although less variant, they remain different after backpropagation. To satisfy the invariance property, we choose to describe each workload by a unique vector $W_j$,  the {\em job level encoding},  by taking the centroid of all instance level encodings. % for job $j$.
%\cut{	
	\begin{equation}\label{eq-centroids}
	W_j = \displaystyle\frac{1}{|I_j|}\displaystyle\sum_{i\in I_j} \bar{E}_j^i
	\end{equation}
%}

{\bf Similarity-preserving}. Finally, we consider the similarity-preserving requirement. 
In the autoencoder approach,  during backpropagation all the fully connected layers are adjusted by all training data. Hence, all the weights in the architecture are shared across the  jobs. In addition, for two similar jobs that have similar observations for each given configuration, our customized cost function in Eq.~\ref{loss-ae} ensures that the bottleneck layer  recovers the same configuration and can reconstruct similar approximate observations. Hence, the chance of having the same invariant encoding in the bottleneck layer is maximized.

%OLD TEXT
%This approach also offers a better way of information sharing between two workloads. It is because during backpropagation, all the fully connected layers including the FC layer whose output is the encoding  are adjusted no matter to which workload the observation belongs. As such, it is more likely to be true that when two workloads are similar, their extracted encodings are similar  as well. 


{\bf Training \& Hyperparameter Tuning.}
Both the autoencoder and the regressor are trained {\em periodically} and {\em offline} from the available training data $T$. To avoid overfitting, important hyper-parameters of the neural network architectures such as the learning rate, the number of hidden layers and the size of each hidden layer, are also tuned via cross-validation~\cite{hastie01statisticallearning}. Such offline training does not affect online performance. When a new job is submitted, we simply run the autoencoder to extract the job level encoding, and use the regressor to predict the latency over a new configuration  upon request of the optimizer, as described in Section 2. 

%\cut{The training of the autoencoder learns all the weights in the neural network so that it can transform observations $O_j$ into workload encodings $W_j$, whereas the training of the regressor aims to learn the function $\tilde{l}_j^i = h^l(W_j, \theta_j^i)$, which  approximates the true latency $l_j^i$. Luckily, both models in this approach can be trained  {\em periodically} in the background, without affecting any running jobs. } 
%
%When a new job $n$ is submitted,  our system performs online operations via both models. First, we use the autoencoder to extract the instance level encoding (which is also the job level encoding given the single configuration see thus far) from the observed trace $T_n^1=(\theta_n^1, O_n^1)$. Then, we use the regressor to predict the latency over a new configuration $\theta_n^2$ upon request of the optimizer.
%When both models are updated in the background training process, we simply switch to use the new models.

%We adopt in this approach a periodic training over submitted jobs and configurations for both the auto-encoder and the regressor. Due to the decoupling between the workload encoding extraction and the regression, the regressor can be any state of the art regressor. For example, it can be a neural network regressor, or an SVM regressor or even a gradient boosting regressor, but it has to be fit on $<W_j, \theta_j^i>$. The regressor has to learn a function $\tilde{l}_j^i = h^l(W_j, \theta_j^i)$ that approximates the true latency $l_j^i$.
%For a new job $k$, submitted to the cloud and for which we want to make predictions, the autoencoder approach allows an online strategy for prediction. First of all, we use the trained autoencoder to extract the instance level encoding (which is the job level encoding too in this case) from the observed trace $T_k^1=(\theta_k^1, O_k^1)$. Then, we use the regressor to  predict the latency over new configurations $\theta_k^2$.



{\bf Optimizations.}
While our design aims to minimize online overhead when a new job arrives, one may wonder whether it comprises accuracy compared to an aggressive retraining approach that includes the trace of each new job immediately into the training. 
While being prohibitively expensive, it adjusts both models to maximize the accuracy for the new job. 
%In Machine Learning terminology, the aggressive approach achieves a low training error rate for the new job, while our period training achieves a test error rate for the previously unseen job which is often larger than the training error rate. 
%In Machine Learning terminology, the aggressive approach achieves a lower test error than the periodic training approach.
We next propose optimizations to approximate the effect of retraining but without incurring its overhead. 

%\textcolor{red}{No matter how good a regressor is, there are always a difference between the training and test accuracy. Training accuracy is always better than test accuracy for the simple reason that the regressor has a better ability to perfectly predict instances over which it was trained. We introduce in this paragraph a first optimization, on the auto-encoder level, that allows us to benefit from a training-like accuracy for a new submitted jobs under some conditions, without even the need of retraining on the observed trace from that job. Then, we introduce another optimization, on the regressor level, that allows to adjust the predictions whenever the model is off due to the lack of data. }

\textsc{Opt1} (Nearest Neighbor Mapping). To improve autoencoder's accuracy for a new job, our idea is to leverage the fact that multiple jobs may belong to the same template, e.g., SQL queries generated from a parameterized template, or clustering tasks based on the same program but with different parameters. Then we can borrow the encoding from a previous job that uses the same template as the new job and has been included in  training, and then make predictions using the borrowed encoding. 
%The algorithm  is described in Algorithm \ref{alg:autoencoder-star}.  

First, when a new job $n$ has its trace available,  the autoencoder extracts the encoding $W_n$. From the training database, we look for workloads belonging to the same template and retrieve the encoding $W_j$ for each of them.
%we look for training instances that belong to the same template and use the same configuration as the new job, and retrieve the encoding  $W_j^i$ for each such training instance.
Then we calculate the euclidean distance between $W_n$ and each $W_j$, and pick the ``nearest neighbor'' job $p$ that minimizes this distance.
% Finally, to decide whether to borrow the encoding from the job $p$,  we use the regressor to calculate a surrogate error, which is equal to the error made on the latency using  $\theta_n^1$ and the borrowed encoding. If this surrogate error is less than an acceptable threshold $\kappa$, then we choose to borrow the encoding $W_p$, which is an average over all training instances from job $p$; otherwise we return the new job's own encoding, $W_n^1$.
%The advantage of this method is that whenever it succeeds in borrowing an encoding from another job, it gives an accuracy comparable to the accuracy obtained in retraining (as job $p$ is already included in  training). 
Whenever such mapping succeeds , it gives an accuracy comparable to the one obtained in retraining  because job $p$ was already included in training.
%but without  the additional cost of retraining.
This optimization leads to a {\bf hybrid method} that combines the benefits of the encoding approach and the nearest neighbor approach as in~\cite{VanAken:2017:ADM}.

\textsc{Opt2} (Regressor Recalibration). 
To improve the regression model for the new job, we augment the  regressor with a wrapper to mitigate its current prediction error. 
The wrapper computes an offset value for the new job as it arrives and uses it to calibrate further predictions. More specifically,   the offset is the error made in the first prediction for the new job, i.e., the difference between the predicted and  true values of the latency ($\tilde{l_n^1} - l_n^1$) for the initial configuration $\theta_n^1$.

%Due to space constraints, we leave the pseudo-code of the above two optimizations to \cite{TR}.

%First, when a new job's trace $T^1_n$ is sent to the autoencoder, it extracts its encoding $W_n^1$. Then, from the training database it looks for other jobs in the same template that use the same configuration as the new job, and extract the encoding from the trace corresponding to that configuration $W_j^i$ (not the averaged one). Afterwards, it calculates the euclidean distance between $W_n^1$ and all other $W_j^i$, and it picks the "proxy" job p, which minimizes this distance. Finally, to decide whether borrowing encoding from the job p makes sense or no, it uses the trained regressor to calculate a surrogate error equals to the error made on the latency (corresponding to the initial configuration $\theta_n^i$ ) using the borrowed encoding. If this surrogate error is less than an acceptable threshold $\kappa$, then it returns the borrowed encoding $W_p$ from job p (\todo{encoding averaged over all possible partial encodings obtained from configurations for job p}) \textcolor{red}{???}, otherwise it returns the original extracted encoding $W_n^i$.
%The advantage of the extended auto-encoder version is that whenever it succeeds in borrowing an encoding from another job, it gives an accuracy with online prediction that is comparable to the accuracy obtained in retraining, but without paying the additional cost of retraining.
%On the other side, the extended regressor represents a wrapper around the trained regressor. This wrapper stores an additional offset value that is initialized at 0 and is set whenever a new job arrives by invoking the \textbf{calibrate} method described in Algorithm \ref{alg:calibration}. The algorithm shows how to use the wrapper to make prediction over a new configuration when a new job arrives. The main idea is to adjust future predictions by taking into consideration the absolute error it makes when it predicts the initial latency. Thus, the value of the offset is the difference between the predicted and the true value of the latency ($\tilde{l_n^i} - l_n^i$) for the initial configuration $\theta_n^i$.
%\todo{Again, why do we need to do this?}


       
%%%%%%%%%OLD TEXT %%%%%%%%%

%\textcolor{red}{The autoencoder approach is an effective way to learn robust workload characteristics and accurate performance objectives separately. Indeed, we decouple the workload extraction part from the regression part as we can see in figure \ref{fig:auto-encoder}. \todo{khaled: add the regression part to the figure}. The whole idea of this approach is centered around the auto-encoder, which is a device capable of doing non linear dimensionality reduction to learn a compact representation of the data. This compact representation is learnt by trying to reconstruct an approximation $\tilde{O}$ of the trace observations $O$ provided as input of the autoencoder. Conceptually, this approach allows a better way of information sharing between two workloads. In fact, when we do backpropagation, all the fully connected layers, including the fc layer whose output is the encoding (bottleneck) are adjusted no matter to which workload the observation belongs. Thus, we expect that when two workloads are similar, their extracted encodings will be similar too. }


%Extracting the workload characteristics can be done as thus: after training an auto-encoder capable of reconstructing the observations, we take the vector at the bottleneck output and consider it as the workload characteristics. 
%However, if we simply extract the encoding as described, then we violate the invariance property of the workload characteristics. This is because the vector we extract will include both the workload characteristics as well as information regarding the configuration that yielded the input observation. For a particular job for which we have different input configurations $\theta_j^i$, $\theta_j^{i+1}$, ... and different observations $O_j^i$, $O_j^{i+1}$, ..., we'll get different workload characteristics $W_j^i$, $W_j^{i+1}, ...$ with high variance among them. To the best of our knowledge, there are no existing auto-encoder architecture that produce invariant encoding for variant input vectors. To mitigate this effect, we make a small modification to the standard auto-encoder architecture and we use the architecture shown in the figure \ref{fig:auto-encoder}. Now, we try to explicitly extract the variant part of the observations $\tilde{\theta}_j^i$ (which should be an approximation of the configuration $\theta_j^i$), with another less variant part that represents the workload characteristics $W_j^i$. We adjust the loss function to include both the reconstruction of the observation (1st term), and the extraction of the configuration (2nd term). 

%For example, we tried to add an intermediate input that represents the exact configuration and we introduced an additional term to the loss function to minimize the variance among different instance level encodings belonging to the same job (a.k.a variation coefficient).This effort didn't improve the way encodings were extracted and has yielded some trivial solutions where the encoding vector was meaningless. 

%However, the autoencoder architecture shown in the figure \ref{fig:auto-encoder} is the harvest of our efforts to extract encodings which are less variant. In this architecture, we break the bottleneck layer into two parts. The first one is a variant part $E^{var}$ that tries to approximate the configuration that induced the input observation. The second part, is however supposed to be an invariant part $E^{invar}$ because it should approximate the workload encoding. While the size of the $E^{var}$ is fixed (= size of configuration vector) , the size of $E^{invar}$ remains of our choice, and we later show that we can choose it along with the other hyper-parameters to meet best performances in the objective modeling.
%To reconstruct the configuration from the optimization, we introduced an additional term (the term multiplied by the $\gamma$ coefficient) to the loss function: 
       

==> modeling_experiments.tex <==
%------------------------------------------------------------
\subsection{Deep Learning for Modeling}
In this section, we compare our embedding and autoencoder approaches to alternatives including PCA and Ottertune~\cite{VanAken:2017:ADM}. %a state of the art technique  for performance modeling. 
We focus on the latency model  as it is more complex than the throughput model. 

%We first give high level comparison between performances of state of the art techniques (PCA, Ottertune) and the modeling performance obtained with our 2 proposed techniques Autoencoder and Embedding. We next give more details on performance results obtained with autoencoder as well as added optimizations that yield the best numbers. We mainly report detailed results on the more complex latency model rather than throughput for which we give the high level performance numbers.

\textbf{Evaluation metric.}
we use the Mean Absolute Percentage Error (MAPE) metric to capture model accuracy:  
%$$\mbox{MAPE} = \displaystyle\frac{100}{m}\displaystyle\sum_{j\in J}\sum_{i\in I_j}\frac{|l_j^i - \tilde{l}_j^i|}{l_j^i}$$
$\mbox{MAPE} = \frac{100}{m}\sum_{j\in J}\sum_{i\in I_j} |l_j^i - \tilde{l}_j^i| / l_j^i$,
where $l_j^i$ denotes the true value of the target, $\tilde{l}_j^i$ denotes the predicted value, and $I_j$, $J$, and $m$ are as defined in Eq.~\ref{loss-embedding-pretraining}.
%$J$ is a set of jobs over which the error is calculated. $I_j$ is the set of configuration numbers over which we made predictions for job $j$, and $m$ is the total number of points over which we compute the error. 
\cut{
To compute MAPE, we partition our 64 workloads (52 SQL-like and 12 ML) as follows: the 6 SQL-like workloads with many job configurations are reserved for bootstrapping the model. For the other 46 SQL and 12 ML workloads,} We call a training setting $LO_j$  where we ``leave out'' job $j$ for testing and use other jobs' traces for training. We define two types (T1 and T2) of errors on the same test job. For T2 error, the model is trained only on the traces of other jobs, while for T1, the model is trained also on 20\% of the traces of the test job. 
Thus, the \textbf{T1 error} reflects the generalization power over {\em unseen configurations of familiar jobs}, while \textbf{T2 error} reflects the generalization power over {\em unseen jobs}.
\cut{By default, we take the average over all leave out jobs, unless noted otherwise.} 

%We use the neural network regressor as the default option due to its flexibility for tuning the optimization objective and robustness for handling continuous values.

%\cut{
%\begin{figure}[t]
%	\begin{center}
%		\includegraphics[scale=.33]{figures2/training-setting}
%		\vspace{-0.1in}
%		\caption{\small Training setting for one left out (LO) job}
%		\vspace{-0.2in}
%		\label{fig: training-setting}
%	\end{center}
%\end{figure}
%
%\textbf{Training Setting}
%The whole dataset of traces consisting of 64 jobs (SQL: 6 intensive and 46 parametrized jobs; ML: 12 jobs) is used in our benchmark experiments. We define what we call a training setting $LO_i$ (Leave out job i), the training setting in which we leave Job i out of the training samples. The purpose of defining such training setting is to emulate the real case scenario where a new job is submitted to cloud (the left out job), and the optimizer will use other jobs data to predict latencies over the new job.
%We define two types of errors: T1 and T2 errors that are evaluated on the same test set ("Test Data" as in figure \ref{fig: training-setting}). The only difference is that for T1, the regressor is trained on "Training Data" and "Training complement" while for T2, the regressor is trained only on "Training Data".
%So \textbf{Type1 error} reflects the generalization power over new unseen configurations from familiar jobs; and \textbf{Type2 error} reflects the generalization power over unseen jobs.
%}


%\cut{
%In experiments 1, 2, 3, and 5, we calculate the errors over each possible test job (out of the 46 SQL jobs and 12 ML jobs) (as shown in figure\ref{fig: training-setting} ) and then we report the average errors obtained over SQL and ML jobs separately. However, in the experiment 4, we train separately over SQL jobs and ML jobs.
%In all our experiments, we use with the auto-encoder approach a neural network based regressor. While we could have used any other state of the art regressor with auto-encoder approach, it turns out that neural network regressor has additional leverage over the other regressors because:
%\begin{itemize}
%	\item It predicts continuous values within the space of features (while gradient boosting regressor for example divides the space into regions where it makes discrete predictions)
%	\item It allows us to customize the loss function. As we'll see in the optimization experiment, it's necessary to introduce an asymmetric loss function for the latency predictor to favor overestimating the latency rather than underestimating it.
%\end{itemize}
%}

%\begin{table}[t]
%	\begin{center}
%		\small
%		\begin{tabular}{|rr|c|c|c|c|}
%			\hline
%			%			\multicolumn{2}{|c|}{} & \textbf{T1} & \textbf{T2} & \textbf{T2-Opt2} & \textbf{T2-Inc} \\
%			%			\hline 
%			%			\hline
%			%			\multicolumn{2}{|c|}{\textbf{Embedding}/SQL } & 9.6\% & - & - &  28.8\%\\
%			%			\hline  			
%			%			\multicolumn{2}{|c|}{\textbf{Embedding}/ML } & 19.6\% & - & - &  21.4\%\\
%			%			\hline \hline
%			
%			\multicolumn{2}{|c|}{\textbf{AE}/SQL } & \textbf{T1} & \textbf{T2-NoOpt}  & \textbf{T2-Inc}  & \textbf{T2-Opt2}\\
%			\hline
%			
%			$\gamma=$ & $0$ & 15.6\% & 32.6\%  & 21.9\% & 21.7\% \\
%			\hline
%%			& $10^{-5}$ & 15.1\% & 29.5\%  & 21.1\% & 21.5\% \\
%%			\hline
%			& $10^{-2}$ & 15.2\% & 28.1\%  & 19.2\%  & 19.1\% \\
%			\hline
%			& $10^{-1}$ & 13.6\% & 29.8\%  & 19.1\%  & 17.5\% \\
%			\hline
%			& $1$ & 13.5\% & 28.4\%  & 17.5\% & 16.8\% \\
%			\hline
%			& $10$ & 14.8\% & 34.3\% & 19.6\%  & 19\%  \\
%			\hline
%			& $100$ & 17.48\% & 42.56\%  & 22.38\% & 21.79\% \\
%			\hline
%%			& $10^5$ & 20\% & 46.1\%  & 26.8\% & 26.5\% \\
%%			\hline
%%			& $10^{10}$ & 23.1\% & 43.6\%  & 31.6\% & 31.8\% \\
%%			\hline
%			
%			\multicolumn{2}{|c|}{\textbf{AE}/ML}  & \textbf{T1} & \textbf{T2-NoOpt} & \textbf{T2-Inc} & \textbf{T2-Opt2}  \\
%			\hline
%			$\gamma=$ & $0$ & 20.9\% & 49.7\%  & 38.3\% & 50.6\% \\
%			\hline
%%			& $10^{-5}$& 21.9\% & 52.3\%  & 40.1\% & 48.9\% \\
%%			\hline
%			& $10^{-2}$ & 18.9\% & 56.6\%  & 48.1\%  & 60.2\% \\
%			\hline
%			& $10^{-1}$ & 16.8\% & 53.9\%  & 45.1\% & 48.2\% \\
%			\hline
%			& $1$ & 16.2\% & 58.8\%  & 45.7\% & 51.9\%\\
%			\hline
%			& $10$ & 17.6\% & 64.6\%  & 49.2\% & 56\% \\
%			\hline
%			& $100$ & 19.87\% & 55.08\%  & 47.13\% & 59.45\% \\
%			\hline
%%			& $10^5$ & 22.1\% & 47.2\%  & 33.5\% & 45\% \\
%%			\hline
%%			& $10^{10}$ & 21.1\% & 39.2\%  & 35.8\%  & 47.2\% \\
%%			\hline
%			
%		\end{tabular}
%		%\vspace{-0.1in}
%		\caption{\small T1 and T2 errors of  Autoencoder with varied $\gamma$. }
%		%\todo{$\gamma=1$ means  92\% of contribution of 2nd term} to the loss function in Eq.~\ref{loss-ae}. 
%		\vspace{-0.4in}
%		\label{table: experiment1-2}
%	\end{center}
%\end{table}

%\cut{
%\begin{figure}[t]
%	\begin{center}
%		\includegraphics[scale=.6]{figures/varying-gamma-sql}
%		\vspace{-0.1in}
%		\caption{\small T1 and T2 errors with different values of  $\gamma$ for SQL workloads. $\gamma = 1$ means  ... of contribution of 2nd term to the loss function in Eq.~\ref{loss-ae}. }
%		\vspace{-0.2in}
%		\label{fig: varying-gamma-sql}
%	\end{center}
%\end{figure}
%
%\begin{figure}[t]
%	\begin{center}
%		\includegraphics[scale=.6]{figures/varying-gamma-ml}
%		\vspace{-0.1in}
%		\caption{\small T1 and T2 errors with different values of  $\gamma$ for ML workloads. $\gamma = 1$ means  ... of contribution of 2nd term to the loss function in Eq.~\ref{loss-ae}. }
%		\vspace{-0.2in}
%		\label{fig: varying-gamma-ml}
%	\end{center}
%\end{figure}
%}

{\bf Expt 1: Tuning of the Autoencoder (AE)}. 
We first perform  experiments to investigate optimizations proposed for our autoencoder (AE) approach. 
We calibrated our customized cost function, in Eq.~\ref{loss-ae}, by tuning its the parameter $\gamma$, 
%which balances the two terms in the total loss. 
and found $\gamma=1$ to work the best. 

%\textit{Customized cost function}.
%%We next illustrate the influence of the hyper-parameter $\gamma$ on both T1 and T2 errors. Then, we present more detailed experimental results that yielded to our final autoencoder results and finally, we compare the autoencoder approach with two baselines.
%We begin  by investigating the new loss function, in Eq.~\ref{loss-ae},  proposed to derive invariant encodings. We varied the parameter $\gamma$, which balances the two terms in the total loss. 
%%The results are shown in figures \ref{fig: varying-gamma-sql} and \ref{fig: varying-gamma-ml} as well as 
%%in Table \ref{table: experiment1-2}.
%The results in Table \ref{table: experiment1-2} show 
%that $\gamma$ that allocates $92\%$ of contribution to the 2nd term of the loss function (approximation error of the job configuration) gives the best performances for both T1 and T2 ($\gamma=1$). 

\textit{Simulating retraining} (OPT2). 
As Table~\ref{table:summary-detailed-modeling} shows, without optimization, the T2 errors of AE are quite high. OPT2  in \S\ref{subsec:autoencoder} calibrates the regressor as approximation of incremental training. When it is applied,  the T2 error for SQL jobs is reduced, but T2 error for ML jobs remains high. 

%With $\gamma$ tuned, the T2 errors of the  autoencoder are still quite high.
%To get a sense of the better performance possible, we  incur incremental training for the regressor using the new trace,  or use the optimization, OPT2 in \S\ref{subsec:autoencoder}, that calibrates the regressor as approximation of incremental training, as shown in the T2-Inc and T2-Opt2 columns. Incremental training or calibration  can indeed reduce errors, but the errors for the ML jobs are still high.


\begin{table}[t]
	\small 
	\begin{center}
		\begin{tabular}{|c||c|c||c|c|}
			\hline
			& \multicolumn{2}{c||}{\textbf{SQL-like Jobs}} & \multicolumn{2}{c|}{\textbf{ML Jobs}} \\ \hline
			
			{\bf Trained on all traces} & \textbf{T1} & \textbf{T2} & \textbf{T1} & \textbf{T2} \\
			\hline
			$Autoencoder (No Opt)$ & 13.5\% & 28.4\%  & 16.2\% & 58.8\% \\
			\hline
			$Autoencoder+Opt2$ &  13.5\% & 16.8\%   & 16.2\% & 51.9\% \\
			\hline
			$Autoencoder+Opt1$ & 16.46\% & 17.19\%  & 4.55\%  & 4.25\% \\%\part{title}
			\hline
%			$Autoencoder+Opt1/2$& 16.46\% & 14.25\%  & 4.55\% & 12.61\% \\
			$Autoencoder+Opt1/2$& 16.46\% & 14.25\%  & 4.55\% & 4.25\% \\

%			\hline \hline
%			{\bf Trained on 50\%  traces} & \textbf{T1} & \textbf{T2} & \textbf{T1} & \textbf{T2} \\
%			\hline
%			$Autoencoder+Opt1/2$ & 16.44\% & 15.70\% & 8.69\% & 9.85\% \\ 
			\hline
			
		\end{tabular}
		%		\vspace{-0.1in}
		\caption{\small  Optimizations of Autoencoder for latency.}
		\vspace{-0.4in}
		\label{table:summary-detailed-modeling}
	\end{center}
\end{table}


%\begin{table}[t]
%	\small 
%	\begin{center}
%		\begin{tabular}{|c||c|c||c|c|}
%			\hline
%			& \multicolumn{2}{c||}{\textbf{SQL-like Jobs}} & \multicolumn{2}{c|}{\textbf{ML Jobs}} \\ \hline
%			
%			& \textbf{T1} & \textbf{T2} & \textbf{T1} & \textbf{T2} \\
%			\hline
%			$Autoencoder (No Opt)$ & 14.03\% & 31.09\% & 17.84\% & 47.98\% \\
%			\hline
%			$Autoencoder+Opt2$ & 14.03\% & 19.26\% & 17.84\% & 46.43\% \\
%			\hline
%			$Autoencoder+Opt1$ & 16.44\% & 19.75\%& 8.69\% & 9.85\%\\
%			\hline
%			$Autoencoder+Opt1/2$ & 16.44\% & 15.70\% & 8.69\% & 15.71\% \\ 
%			\hline
%		\end{tabular}
%		%		\vspace{-0.1in}
%		\caption{\small  Summary of T1 and T2 errors for latency with partial training settings.}
%		%		\vspace{-0.4in}
%		\label{table:summary-detailed-modeling-partial}
%	\end{center}
%\end{table}

\textit{Borrowing encodings} (OPT1). 
We next add OPT1, which for a new job borrows the encoding from a similar job that belongs to the same template and has been included in training. %, as described in \S\ref{subsec:autoencoder}.
As Table~\ref{table:summary-detailed-modeling} shows, 
 ML jobs benefit from the optimization more than SQL jobs because they are similar to each other. 
 OPT1 allows the regressor to predict for a new encoding without interpolating in the (sparse) space of encodings,  but using a  borrowed encoding already in the training data. 
%For the T2 error, without OPT1 the regressor makes predictions for a new encoding by interpolating in the (sparse) space of encodings  through the values it has learned. With OPT1, it does not have to do such interpolation since the borrowed encoding exists in the training already. 

To combine OPT1 and OPT2, we use an adaptive scheme: using OPT1 we map the new job to a past job via the encoding. If the model  of the past job can predict the performance of the new job under the current configuration within 10\% from the observed value, we use OPT1 alone; otherwise, we apply OPT2. %This is because OPT2 aims to  simulate incremental training and does not always offer stable performance. 
This  scheme, denoted as OPT1/2, 
keeps the errors around 16\% or less for SQL jobs and 5\% for ML jobs. 
 

%We compare the normal autoencoder with the extended autoencoder ($autoencoder*$). The former simply extracts the encoding for the new job from the trace that is provided and returns the encoding. The latter, however, borrows an encoding from a similar job.
%(1) ML jobs benefit from the optimization more than SQL jobs because ML jobs are very similar to each other. 
%(2) Compared to the numbers of autoencoder in Table~\ref{table:experiment3},  OPT1 makes a significant improvement. 
%Without OPT1, the regressor tries to make predictions using a complete new encoding by interpolating in the space of encoding dimensions through encoding values it has learned. However, with OPT1 the regressor does not have to do such interpolation since the borrowed encoding exists in the training setting. Since the space spanned along the encoding dimensions is sparse (e.g., only 64 different encodings) the interpolation comes with a huge error.

%-------------------------------------------------------------------------------


%\todo{add footnote for autoencoder numbers: For SQL workloads, both Opt1 and Opt2 have been used with autoencoder to get best results, while for ML workloads, only Opt1 was used}


\textbf{Expt 2: Comparison to Others}.
We next compare AE to the embedding approach,  PCA, and Ottertune~\cite{VanAken:2017:ADM}. 
%The results are shown in Table~\ref{table:summary-modeling}.

%OLD TEXT
%The autoencoder approach outperforms, in both online and offline performance modeling scenarios, other classical ML techniques such as PCA, as well as state of the art tuning tools such as Ottertune. Furthermore, we learn that the proposed embedding approach can be promising in the offline scenario (T1 error), whenever we have enough bootstrapping workloads (which is the case for SQL workloads) in our training set.
%
%We first explain why the autoencoder performs better than other state of the art approaches, and then we explain why the Embedding approach for deriving the latency model did not work well.
%The results  are shown in the Table  \ref{table:summary-modeling}.
%The power of the autoencoder approach mainly lies in its ability to provide a workload encoding vector for  each new job whenever its trace becomes available. This allows the autoencoder to gather knowledge from multiple workloads trained on different configurations, and then leverage this knowledge whenever it wants to predict objective values for the new job. This approach achieve error values as low as 14.25-16.46\% for SQL jobs, and 4.25\%-4.55\% for ML jobs. Note that ML errors are less than errors obtained with auto-encoder because all workloads in our ML benchmark achieve similar performances.

\cut{
The power of the autoencoder approach lies in its ability to provide a workload encoding for  each new job whenever its trace becomes available. This allows the autoencoder to gather knowledge from past jobs trained on different configurations, and then leverage this knowledge whenever it wants to predict objective values for the new job. 
}

1) \textit{Embedding}: As Table~\ref{table:summary-modeling} shows, 
the Embedding approach achieves decent T1 errors for familiar jobs, but higher T2 errors for unseen jobs. When a new job is submitted, Embedding triggers incremental training with the new trace to construct its embedding vector. However, it does not offer stable performance in T2 error, %for SQL and ML jobs, 
which is known due to the increased chance of being stuck at local optima. 
%\todo{explain why in the embedding it's not a good idea to map a new workload to a previously seen workload...}
In addition, the encoding of a new job is learned only from the latency numbers (not all runtime metrics), and with limited sharing with the past jobs, hence not as accurate as autoencoder.
%making it hard to transfer information between the past jobs to the new job.

%{\color{red} even if we're stuck at a local optima, after incrementally optimizing to an existing workload, why didn't we try to borrow an encoding using the embedding approach???}

2) \textit{PCA}: We use PCA to transform the runtime metrics to an encoding of a small size for each job. Then we use  the neutral network (NN) regressor  for prediction as in our autoencoder approach.
PCA incurs higher errors  than  autoencoder because PCA performs \textbf{linear} projection of the  vector  of runtime metrics on axes maximizing the variance. In contrast, autoencoder performs non-linear transformation to construct workload encodings and thus can model more complex workload characteristics. Even if we include OPT2 to improve its prediction for unseen jobs, its T2 error reduces to 21.6\% for SQL and 66.2\% for ML jobs, still much worse than the performance of the autoencoder.

\begin{table}[t]
	\small 
	\begin{center}
		\begin{tabular}{|c||c|c||c|c|}
			\hline
			& \multicolumn{2}{c||}{\textbf{SQL-like Jobs}} & \multicolumn{2}{c|}{\textbf{ML Jobs}} \\ \hline
			& \textbf{T1} & \textbf{T2} & \textbf{T1} & \textbf{T2} \\
			\hline
			\textbf{Autoencoder} & 16.46\% & 14.25\%  & 4.55\% & 4.25\% \\
			\hline
			\textbf{Embedding} & 9.6\% & 28.8\% & 19.6\% & 21.4\% \\
			\hline
			\hline
			\textbf{PCA + NN}  & 19.8\% & 56.6\% & 26.6\% & 77.1\% \\ %without any of the optimizations
			\hline
			\textbf{PCA + NN} (Opt2)  & 19.8\% & 21.6\% & 26.6\% & 66.2\% \\ %Numbers here show T2 with calibration (with opt2)
%			\hline
%			\hline
%			\textbf{Ottertune}~\cite{VanAken:2017:ADM}& 29.03\% & 27.93\% & 75.99\% & 76.43\% \\
			\hline	
			
		\end{tabular}
		%		\vspace{-0.1in}
		\caption{\small  T1 and T2 errors using Embedding and PCA.}
		\vspace{-0.2in}
		\label{table:summary-modeling}
	\end{center}
\end{table}


3) \textit{Ottertune}: Ottertune is a state of the art technique for performance modeling using a blackbox approach. 
In essence, it takes a {\bf nearest neighbor} approach to map a new job to a closest past job by a customized similarity metric, and trains a regression model using configurations from the new job and the  nearest neighbor to predict the performance  for the new job. Our implementation is given in Appendix~\ref{appendix:model-results}.
%Ottertune fails to accurately predict the latency over new jobs in both online and offline modes, whether we observe 1 or more traces of the workload into consideration. We can see that error rates it provides are double the ones obtained with the auto-encoder approach for SQL workloads, and for ML workloads are 16x higher than errors obtained with the auto-encoder approach.
Table~\ref{table: autoencoder-ottertune-comparison} compares autoencoder and Ottertune under different training settings. We denote by \textit{Full} the training setting in which we use all data from past jobs when doing both the workload mapping and regressor's performance evaluation. So all prior results are provided for the full training. \textit{Partial}-50\% (30\%) refers to a training setting in which we use only 50\% (30\%) of the configurations we have for past jobs. 
%For \textit{Partial2} we drop 70\% of the configurations of past jobs. 
%While Ottertune's workload mapping module can do a great job in finding the most similar workload, its main pitfall lies in the fact that its predictive module (which uses Gaussian Processes) doesn't leverage all traces it has in its training data. This is because it doesn't create an encoding of the workload so that it can jointly train a regressor on traces coming from multiple workloads. This lack of knowledge transfer among different workloads in Ottertune yields higher error than errors obtained with our architecture when each past job have only few configurations.

For autoencoder,  even if we reduce the training data by dropping $70\%$ of the configurations of past jobs,  autoencoder maintains the errors within 19\%  for SQL and ML jobs. 
For Ottertune, it appears to have good performance with full training, but profiling shows that the good performance is due to the artifact  that our workloads are sampled with similar configurations. When Ottertune maps a new job $n$ to a past similar job $p$, the test configurations of $n$ are almost the same as those of $p$. 
Once we reduce the overlapping configurations between jobs, as in partial training, the errors of ML jobs grow much faster than those of SQL jobs with Ottertune. The reason is that in our dataset, 
 SQL jobs exhibit small variance in latency under different configurations, so Ottertune can achieve lower errors. However, ML workloads exhibit a larger degree of variance in latency, so Ottertune's error  increases up to 60\%   with reduced overlap in configurations. 

\begin{table}[t]
	\small 
	\begin{center}
		\begin{tabular}{|c||c|c||c|c|}
			\hline
			& \multicolumn{2}{c||}{\textbf{SQL-like Jobs}} & \multicolumn{2}{c|}{\textbf{ML Jobs}} \\ \hline
			
			 & \textbf{T1} & \textbf{T2} & \textbf{T1} & \textbf{T2} \\
			\hline
			$AE/Full$ & 16.46\% & 14.25\%  & 4.55\% & 4.25\% \\
			\hline
			$AE/Partial-50\%$ & 16.44\% & 15.7\%  & 8.69\% & 10.12\% \\
			\hline
			$AE/Partial-30\%$ & 18.72\% & 18.04\%  & 18.7\% & 17.23\% \\
			\hline \hline
			$Ottertune/Full$ & 8.05\% & 9.12\%  & 8\% & 5.26\% \\
			\hline
			$Ottertune/Partial-50\%$ & 14.86\% & 14.39\%  & 29.72\% & 19.71\% \\
			\hline
			$Ottertune/Partial-30\%$ & 21.23\% & 19.29\%  & 60.51\% & 41.43\% \\
			\hline
			
		\end{tabular}
		%		\vspace{-0.1in}
		\caption{\small  Errors obtained with Autoencoder and Ottertune under different training settings.}
		\vspace{-0.4in}
		\label{table: autoencoder-ottertune-comparison}
	\end{center}
\end{table}

%\begin{table}[t]
%	\small 
%	\begin{center}
%		\begin{tabular}{|c||c|c||c|c|}
%			\hline
%			& \multicolumn{2}{c||}{\textbf{SQL-like Jobs}} & \multicolumn{2}{c|}{\textbf{ML Jobs}} \\ \hline
%			
%			& \textbf{T1} & \textbf{T2} & \textbf{T1} & \textbf{T2} \\
%			\hline
%			$AE/Full$ & 16.46\% & 14.25\%  & 4.55\% & 4.25\% \\
%			\hline
%			$AE/Partial-50\%$ & 16.44\% & 15.7\%  & 8.69\% & 10.12\% \\
%			\hline
%			$AE/Partial-30\%$ & 18.72\% & 18.04\%  & 18.7\% & 17.23\% \\
%			\hline
%			$Ottertune/Full$ & 9.96\% & 11.5\%  & 7.61\% & 7.4\% \\
%			\hline
%			$Ottertune/Partial-50\%$ & 19.56\% & 19.29\%  & 47.72\% & 38.42\% \\
%			\hline
%			$Ottertune/Partial-30\%$ & 26.16\% & 25.47\%  & 75.48\% & 62.02\% \\
%			\hline
%			
%		\end{tabular}
%		%		\vspace{-0.1in}
%		\caption{\small  Comparison between errors obtained with Autoencoder and Ottertune under different training settings.}
%		\vspace{-0.4in}
%		\label{table: autoencoder-ottertune-comparison}
%	\end{center}
%\end{table}


%Reasons:
%1) nearest workload
%2) training a model using only the new job and the nearest neighbor
%3) difference in regressor


%%Before optimization
%%gamma, contribution of obs to loss function, contribution of conf to loss function
%0.01 89.28571428571428 10.714285714285714
%0.1 45.45454545454545 54.54545454545454
%1 7.6923076923076925 92.3076923076923
%10 0.8264462809917356 99.17355371900827
%100 0.08326394671107411 99.91673605328893
%%After optimization
%%gamma, contribution of obs to loss function, contribution of conf to loss function
%0.01 38.75965324493811 61.240346755061886
%0.1 12.773183798310928 87.22681620168906
%1 4.102206510256064 95.89779348974393
%10 0.9205789269375461 99.07942107306245
%100 0.21474624232373155 99.78525375767627


{\bf Expt 3}: For the 4D dataset, due to reduced dimensionality, our autoencoder approach achieved T1 and T2 errors within 8.5\% for SQL jobs and within 3.6\% for ML jobs. Additional details are given in Appendix~\ref{appendix:results}.

{\bf Expt 4}: Throughput modeling is easier than latency because for most configurations the throughput is strongly affected by the input rate. Overall,  we achieve T1 error of 0.21\% and T2 error of 0.32\% on the average for SQL jobs, and  T1 of 0.28\% and T2 of 0.34\% for ML workloads.


\cut{
\textbf{Summary.}
Table \ref{table:summary-modeling} summarizes the major results in modeling. Our optimization methods, OPT1 and OPT2, offer remarkable improvement of the autoencoder, resulting in around 14.2\%-16.5\% errors for both T1 and T2 for SQL-like jobs, and 4.2\%-4.5\% errors for ML jobs.
{\color{red} How can we explain that for SQL workloads in offline mode (T1) Opt1 is increasing the error rate?}
We can conclude mixing both optimization strategies yield better results whenever there are room for improvement. Yet, the calibration sometimes may incur extra error because of its readiness to induce overfitting on the unique seen trace.
% We have verified indeed that our first optimization strategy improves results for both T1 and T2 errors, while the second optimization improves results for T2 error only.
}




==> optimization.tex <==
\section{Theoretical Foundation}

\label{sec:optimizer}
In this section, we present a theoretical foundation for solving a multi-objective optimization problem, which allows us to design fast algorithms in the next section. 
%we design a multi-objective optimizer when the predictive models for user objectives are given.\cut{We will defer the discussion of modeling to the next section.}  

%In this section, we first give the formal definition of a Multi-Objective Optimization and discuss various aspect regarding it. Then we describe how to build the skyline efficiently. Last, we discussion the automatic execution plan selection issue.

%------------------------------------------------------------------
\subsection{Problem Statement}
\label{subsec:moo_problem}
We begin with a mathematical definition of the multi-objective optimization problem for a given user task.
% which is also known as vector optimization as follows.

{\problem{\textbf{Multi-Objective Optimization (MOO).}
\begin{eqnarray}
\label{eq:mult_obj_opt_def}
  \arg \min_{\bm{x}} &f(\bm{x})=& {\left[
        \begin{array}{l}
          F_1(\bm{x}) = \Psi_1(\bm{x}) \\ %-\lambda
          F_2(\bm{x})= \Psi_2(\bm{x}) \\
%          F_3(\bm{x})= -c*S\\
          ...\\
          F_k(\bm{x}) = \Psi_k(\bm{x}) 
        \end{array}
      \right]} \\
 \nonumber s.t. & &  {\begin{array}{l}
%          \lambda > 0 \\
          \bm{x} \in \Sigma \subseteq \mathbb{R}^d  \\ %|\bm{x}|=d
          F_i^L \leq F_i(\bm{x}) \leq F_i^U, \,\,\, i=1,2,...,k\\
%    {\color{red}     g_j(\bm{x}) \leq 0, \,\,\, j=1,2,...,m }\\
%     {\color{red}    h_l(\bm{x}) = 0, \,\,\, l=1,2,...,e }\\
        \end{array}}
\end{eqnarray}
}}\noindent{where $\bm{x}$ is the job configuration with $d$ parameters,   
$\Sigma \subseteq \mathbb{R}^d$ denotes all possible job configurations. 
Further, $F_i(\bm{x})$ generally denotes  one of the $k$ objective functions,  while  $\Psi_i(\bm{x})$  refers particularly to the predictive model learned for this  objective. % based on $\bm{x}$ and $W$. 
If a task objective favors larger values,  we add the minus sign to the objective function to transform it to a minimization problem. Optionally, there can be a number of inequality constraints on the parameter vector, $\bm{x}$. 
%inequality constraints and equality constraints on the parameter vector, $\bm{x}$, as in general optimization problems.
%We will use $f$ instead of $f(\bm{x})$ when its meaning is clear in the context. 
Note that our problem involves the the $d$-dimensional {\bf parameter space}, $\Sigma$, and the $k$-dimensional {\bf objective space}, $\Phi$, where each dimension corresponds to an objective. }

In general, the multi-objective optimization (MOO) problem leads to a set of solutions rather than a single optimal solution. Then the notion of optimality in the MOO setting is based on the following concepts:
%\textcolor{red}{In the single-objective optimization task, there exists a total order, and the goal is to find the minimum element (feasible solution) under this total order. Hence reduce the result of interest to single element. Unfortunately, in the multi-objective optimization case, there does not exist such a total order. For example, for tuple $(3,6)$ and $(4,5)$, they are not comparable by $\leq$ relationship in absolute sense. In response, instead of seeking single minimum element, one can try to reduce the result of interest as much as possible. It means that if there exists a partial order, then every element which is not a minimal can be safely removed from the result. In this case, the multi-objective optimization can return all the minimal elements.}
%\textcolor{red}{There exists a partial order satisfying our requirement:}

\definition{\textbf{Pareto Domination:} In the objective space $ \Phi$, a point \bm{$f'$} Pareto-dominates another point \bm{$f''$} iff $\forall i \in [1, k], f_i' \leq f_i''$  and $\exists j \in [1, k], f_j' < f_j''$.
%\definition{\textbf{Pareto domination:} A point $x_1 \in \Sigma$ Pareto-dominates another point $x_2 \in \Sigma$ iff $\forall i, F_i(x_1) \leq F_i(x_2)$  and $\exists j, F_j(x_1) < F_j(x_2)$.


\definition{\textbf{Pareto Optimal:} In the objective space $\Phi$, a point \bm{$f^*$} is Pareto optimal iff there does not exist another point \bm{$f'$} that Pareto-dominates it.

\definition{\textbf{Pareto Set (Frontier):} For a given job, the Pareto set (frontier) $\mathcal{F}$ includes all the Pareto optimal points in the objective space $\Phi$, and is the solution to the MOO problem. \cut{We refer to  a Pareto  optimal point  as a {\em reference point}, $F^0_i$, if it achieves the minimum for the objective $f_i$.}


%\vspace{0.1in}
The MOO problem  is characterized by a mapping ($\Psi_1, \cdots \Psi_k$)  from the numerical parameter space, $\Sigma$, to the numerical objective space, $\Phi$. Through this mapping, we want to find those configurations  in the parameter space  $\Sigma$ that lead to Pareto-optimal points in the objective space $\Phi$.

Besides the above definition, we impose performance requirements   to suit the needs of a multi-objective optimizer for cloud analytics. As noted in Section 1, the Pareto frontier needs to be computed with {\bf good coverage} in order to enable recommendations of best configurations,  and {\bf high efficiency}  to respond to the need of starting a new database instance or adapt to bursty data loads quickly in the serverless database case, or to reduce the delay of starting a recurrent workload at a scheduled time. 

%In addition to the above definition, we impose the following performance requirements  for the MOO approach to suit the needs of an optimizer for cloud data analytics:
%
%{\bf Coverage of the Pareto Frontier}:  Since the Pareto frontier is computed to recommend a new configuration that best explores tradeoffs between different objectives, it should provide good coverage of the overall objective space. Further, it should provide coverage in  fine resolution for the regions when the tradeoffs are significant, e.g., for a region where the Pareto frontier exhibits a sharp turn, meaning that a small compromise of one objective will lead to significant improvement of another objective. 
%%As we shall show later in the paper, classical MOO algorithms often fail to provide good coverage of the Pareto frontier~\cite{marler2004survey} or fine resolution for significant tradeoffs~\cite{marler2004survey}.
%
%{\bf Efficiency}: 
%Since our optimizer takes models of task objectives, ($\Psi_1, \Psi_2, \ldots, \Psi_k$), from a machine learning tool, it has to prepare for frequent updates of such models (as new training data becomes available). Before running a user task, the learned models may have changed and the optimizer has to recompute the Pareto frontier in order to make recommendations.   Therefore,  the speed of computing the Pareto frontier is crucial for adapting quickly to bursty workloads  (in the serverless database case) or reducing the delay of starting a recurring workload at a scheduled time. 
%%Most existing MOO algorithms including Weighted Sum~\cite{marler2004survey}, Normal Constraints~\cite{marler2004survey}, Evolutional Methods~\cite{Emmerich:2018:TMO} are not designed to meet such  efficiency requirements.



%------------------------------------------------------------------------------
\subsection{Existing Numerical MOO Methods}
\label{subsec:moo_survey}
%The MOO problem in our setting is characterized by a mapping from the numerical parameter space, $\Sigma$, to the numerical objective space, $\Phi$. Through this mapping, we want to find those configurations  in the parameter space  $\Sigma$ that lead to Pareto-optimal points in $\Phi$. 
%Since it is infeasible to enumerate through the {\em infinite} set of configurations in $\Sigma$, the solution is less likely to be a combinatorial one as in SQL databases~\cite{Ganguly:1992:QOP,Kllapi:2011:SOD,Trummer:2014:ASM,TrummerK15}. Instead, we take a numerical approach, for which there exist three popular methods: 

%MOO for SQL queries~\cite{Ganguly:1992:QOP,Kllapi:2011:SOD,Trummer:2014:ASM,TrummerK15} usually takes a combinatorial approach: It examines a {\em finite} set of query plans based on relational algebra, and selects the Pareto-optimal ones based on estimated costs of each plan. Since query plans share common substructures, the solution lies in how to efficiently search through (a subset of) these query plans and find the (approximate) Pareto-optimal plans. Such a procedure that searches over a finite structure is formally grounded in combinatorics. 
\cut{
MOO for SQL queries~\cite{Ganguly:1992:QOP,Kllapi:2011:SOD,Trummer:2014:ASM,TrummerK15}  examines a {\em finite} set of query plans based on relational algebra, and selects the Pareto-optimal ones based on estimated costs of each plan. Since the optimization problem in our setting requires searching through an infinite paragraph space, $\Sigma$, the solution is unlikely to be a combinatorial one as in SQL optimization. Instead, we take a numerical approach, for which there exist three popular MOO methods in the literature: 
}

\underline{Weighted Sum (WS)}~\cite{marler2004survey}. 
%Known as vector optimization, the MOO problem in our setting is hard to solve directly.  A common method for solving this problem is the Weighted Sum (WS) method~\cite{marler2004survey}.
The WS method~\cite{marler2004survey}
transforms the MOO problem into a single-objective optimization problem by distributing the weights (preferences) among different objectives.
% However, without knowing the actual user preference each weight distribution is only a guess. 
The WS method tries a number of weight distributions and for each computes the optimal solution. It returns the collection of solutions as the Pareto set. 
%$F(\bm{x}) \subseteq \mathbb{R}^k$
A major issue with WS  is the {\bf poor coverage} of the Pareto frontier~\cite{das1997a, messac2012from}, which is undesirable if one wants to understand tradeoffs across the entire Pareto frontier.
%Each solution in the Pareto Optimal set can be mapped to a point, $y \in \mathcal{F}$, on the Pareto frontier based on the values of the objectives achieved.
%If one wishes to construct the Pareto frontier by the WS method, 
%One would hope that the collection of weight distributions used in WS will lead to an even distribution of points on the Pareto frontier. Unfortunately, this is not true.  
%The solutions returned by different weight distributions are often clustered in a small region of the frontier, i.e., having similar values across all objectives, while other parts of the frontier are not covered. This is undesirable if one wants to understand tradeoffs across the entire Pareto frontier.

%In summary, the WS method has the limitation that it may not result in an even distribution of Pareto optimal points and an accurate, complete representation of Pareto Frontier~\cite{das1997a}.
\cut{
It is also known that WS is not able to obtain points on non-convex portions of the Pareto Frontier \todo{in the criterion space}~\cite{das1997a, messac2012from}.
Adaptive Weighted Sum (AWS) approach, which is a variant of weighted sum approach could handle non-convex function by recursively calling weighted sum approach for the segment which does not have any solutions returned. AWS has much longer running time than WS since WS is invoked many times.
}

\underline{Normalized Constraints (NC)}~\cite{marler2004survey}. To address the coverage issue, the NC method~\cite{messac2003nc} provides a set of evenly spaced Pareto optimal points on the frontier $\mathcal{F}$. %in regarding the Reference points.
It divides the objective space into an evenly distributed grid and probes the grid points to have even coverage of the objective space. 
However, NC suffers from  {\bf efficiency} issues. 
First, it uses a pre-determined parameter, $N^p$, to specify how many Pareto  points  to explore, which can grow exponentially with with the dimensionality of $\Phi$. This parameter can impose high computational cost (if set too high) or produce inaccurate Pareto frontiers (if set too low).
%Controlling the tradeoff between the coverage of the frontier and computation cost, this parameter is hard to set a priori. If this parameter is set too high, the computation cost is high; if it is too low, the Pareto frontier is not accurate.  To have good coverage of the frontier, this parameter grows exponentially with the dimensionality of $\Phi$, making it hard to choose an appropriate number to balance accuracy and efficiency. 
Second, NC is not an incremental algorithm: if  the Pareto frontier built form $k$ probes does not provide sufficient information about the tradeoffs, then the next run with  $k' (> k)$ of probes will start the computation from scratch. 
%\cut{Third, it does not leverage the information already available in the frontier; for example, some region of the frontier is flat and will not gain new information with additional points, whereas another region includes a sharp turn and hence needs more points to better characterize the turning point. 
%Fourth, the solutions returned by NC are not guaranteed to be Pareto optimal. Hence, an additional filter is needed to remove nonviable solutions, resulting in a (much) smaller number of Pareto optimal points returned than $N^p$, as we will show in experiments.}
%Third, the results returned by NC are not guaranteed to be Pareto optimal. Hence an additional filter is needed to ensure the Pareto optimality. 

\underline{Evolutionary Methods} (Evo)~\cite{Emmerich:2018:TMO}
 are randomized methods  to approximately compute the frontier set. 
%\todo{Fei: Add a few sentences. Take comments from the survey.}
As evolutionary methods are used to build an optimizer in our setting, they suffer from two issues:
First, it is not an incremental algorithm. Like the NC method, if  the Pareto frontier built from $k$ probes does not provide sufficient information about the tradeoffs, then the next run with $k' (> k)$ probes will start  from scratch. Since the optimizer does not know the sufficient number of probes in advance, it needs to start from a smaller value and try larger values if more information is needed. Hence, evolutionary methods will suffer from the {\bf efficiency} issue by not being able to reuse the previous result.   
Second, a more severe problem is {\bf inconsistency}: The Pareto frontier built from $k'$ probes can be inconsistent with that built from $k$ probes, as our experimental results show. This causes a major problem in  recommending configurations: if the optimizer uses the Pareto frontier from $k$ probes to make a recommendation due to stringent time requirements, it can be invalidated completely later as the Pareto frontier is recomputed to include more points. 


%FEI's TEXT VERSION 1
%However, there are several drawbacks with the NC method. 
%Firstly, it has a pre-determined parameter, which can be interpreted as how many Pareto optimal points one want to explore. If this parameter is set too high, then the cost is high; if too low then the Pareto Frontier is not accurate. This parameter is exponential with the dimension makes it is hard to control. To make it worse, NC is not an incremental algorithm, if the user not satisfied with the current result, then the next run will start from scratch. 
%
%Secondly, the quality of the Pareto Frontier is not guaranteed to improve providing more Pareto optimal points explored. We will further exhibit this in our experiment section. Intuitively, this means that the even distribution may miss the Pareto optimal points corresponding to the sharp turns in the Pareto Frontier. And these Pareto optimal points can provide more information in demonstrating the Pareto frontier.
%
%Thirdly, the results returned by NC is not guaranteed to be Pareto optimal. Hence an extra procedure (filter) is needed to make sure the Pareto optimality. 

%FEI's TEXT VERSION 1
%WEIGHTED SUM is a common method used in providing a solution to a Multi-objective optimization problem. It transforms the MULTI-OBJECTIVE OPTIMIZATION problem into a single-objective optimization problem by distributing the weights (preference) among different objectives. The issue is that weight distribution is a subjective manner. Without knowing the actual user preference, the weight distribution used in WEIGHTED SUM is just a guess, and this guess will have severe impact on the quality of the solution returned which is often undesirable.
% 
%Another issue is regarding the pareto frontier construction. We will formally define pareto frontier later, for now one can assume that is a set of solution to the MULTI-OBJECTIVE OPTIMIZATION problem. If one wish to construct the pareto frontier by WEIGHTED SUM method, e. g, provide a set of weight distribution and solve corresponding optimization issue. It is often the case multiple optimization problems constructed by different weight distributions will return same solution. This is also undesirable.
 
 %ZHAO's OLD TEXT
%One of the most common approaches to multi-objective optimization is the weighted sum (WS) method \cite{marler2004survey}. However, it is known that WS is not able to obtain \todo{points on non-convex portions of the Pareto optimal set in the criterion space}~\cite{das1997a, messac2012from}. Therefore, WS may not result in an even distribution of Pareto optimal points and an accurate, complete representation of Pareto optimal set~\cite{das1997a}.
%Adaptive Weighted Sum (AWS) approach, which is a variant of weighted sum approach could handle non-convex function by recursively calling weighted sum approach for the segment which does not have any solutions returned. AWS has much longer running time than WS since WS is invoked many times.



%---------------------------------------------------------------------------------
\subsection{Overview of Our Approach}
\label{subsec:progressive}

To meet the aforementioned performance requirements, we introduce a new approach, called {\bf Progressive Frontier}. It incrementally transforms the MOO problem into a series of constrained single-objective optimization problems, which can be solved individually. 
In this section, we prove the correctness of this approach. 
% sharing the same structure but with varied constraints. 
%Then we prove that each solution to these constrained problems is Pareto optimal for the original MOO problem when the Pareto frontier is continuous. 
%Afterwards, we present an algorithm that determines the next set of constrained optimization problems to solve as we expand the Pareto frontier incrementally.
%We begin by presenting the critical part of our approach, i.e., how to transform the MOO problem into solving constrained optimization problems, for which good solvers exist.
We first assume the continuous property of the Pareto frontier and provide the following statements.
We will relax the assumption at the end of the section. 
\todo{Fei: simplify this section}

%OLD TEXT
%To meet the above requirements, we introduce a new approach, called {\bf Progressive Frontier}, that transforms the MOO problem into a set of constrained single-objective optimization problems.
%% sharing the same structure but with varied constraints. 
%Then we prove that each solution to these constrained problems is Pareto optimal for the original MOO problem when the Pareto frontier is continuous. 
%Afterwards, we present an algorithm that determines the next set of constrained optimization problems to solve as we expand the Pareto frontier incrementally.
%We begin by presenting the critical part of our approach, i.e., how to transform the MOO problem into solving constrained optimization problems, for which good solvers exist.
%We first assume the continuous property of the Pareto frontier and provide the following statements.
%We will discuss the extension to more general cases at the end of the section. 
%%Under the continuous frontier assumption, we have the following statements:

	%This is a reasonable assumption for big and fast data analytics systems. Indeed it is about the trade-off of conflicting objectives, worsen performance in one objective would lead to better performance in the other. Otherwise, either there is an overall best plan or the system already go to the extreme case (such as one objective is as large as possible).

\minip{A Single Constrained Optimization Problem.} We begin our solution by trying to generate a single Pareto optimal point through solving a constrained optimization (CO) problem. Our approach overcomes limitations of  traditional CO by automatically choosing the constraint threshold and incrementally improving it while also exploring tradeoffs when computing a solution.

{\problem{\textbf{Constrained Optimization (CO).} Given the MOO defined in Formula~\ref{eq:mult_obj_opt_def}, its constrained optimization  is a single objective optimization problem $P_{\mathcal{C}}^{(i)}$ defined as:
\begin{equation}
\begin{aligned}
\bm{x}_{\mathcal{C}} = \hspace{0.2cm} & \underset{\bm{x}}{\text{\bf arg min}}\hspace{0.3cm}F_i(\bm{x}) ,\\
 \text{\bf subject to}\hspace{0.4cm} & F_j(\bm{x}) \leq \mathcal{C}_j, \hspace{0.1cm} j \in [1,k], j \neq i
\end{aligned}
\label{eq:opt}
\end{equation}
}where $\mathcal{C}_j$ is constraint on the $j$-th objective ($j \neq i$), $\mathcal{C}^{\neg i}=\{\mathcal{C}_j \ | \ j \in [1,k], j \neq i \}$ is the set of constraints on all the objectives except the $i$-th objective.}

{\lemma{For any $m$-th objective of Formula~\ref{eq:mult_obj_opt_def}, its objective value is strictly decreasing when the $n$-th objective $(m\neq n)$ increases, while the values of the other $k-2$ objectives are fixed.}
\label{prop:strict_decreasing}}
\begin{proof}
	Let \bm{$f'$} and \bm{$f''$} be two Pareto optimal points, where $f_l' = f_l''$ if $l \ne m$ and $l \ne n$. Suppose that $f_m' > f_m''$, and  $f_n' \geq f_n''$. Then \bm{$f''$} Pareto dominate \bm{$f'$}, so \bm{$f'$} is not Pareto optimal.
\end{proof}

%All proofs in the paper are given in Appendix~\ref{appendix:opt}.
%left to our tech report~\cite{TR}.

{\proposition \label{prop:equa_constraint} The optimal solution of a constrained optimization problem is achieved when equalities are reached for all the constraints: $F_j(\bm{x}) = \mathcal{C}_j, \hspace{0.1cm} j \in [1,k], \hspace{0.1cm}j \neq i$.}
\begin{proof}
	For any constraint $F_l(\bm{x}) < \mathcal{C}_l$, one can find a $\bm{x}'$ such that all the  $F_l(\bm{x}') = \mathcal{C}_l$ and $F_j(\bm{x}) = F_j(\bm{x}')$ other than $l$ and $i$ . The continous condition guarantees that this is always applicable.  Lemma \ref{prop:strict_decreasing} guarantees that $F_i(\bm{x}') < F_i(\bm{x})$.
%	\todo{?}
\end{proof}

{\proposition  \label{prop:dual_optimal} For a constrained optimization problem $P_{\mathcal{C}}^{(i)}$ and its optimal solution \bm{$f^*$}, form another $P_{\mathcal{C}}^{(l)}$ by switching the roles of $F_i(\bm{x})$ and $F_l(\bm{x})$ while keeping other constraints the same. Then \bm{$f^*$} is the optimal solution to $P_{\mathcal{C}}^{(l)}$.}
\begin{proof}
	$P_{\mathcal{C'}}$ tries to minimizes $F_l(\bm{x})$ under the constraints $F_i(\bm{x}) \leq f_i^*$. By Proposition \ref{prop:equa_constraint}, when $F_i(\bm{x}) = f_i^*$, $F_l(\bm{x})$ achieves its minimium: $F_l(\bm{x}) = f_l^*$. This implies that \bm{$f^*$} is also the optimal solution to $P_{\mathcal{C'}}$.
%	\todo{?}
\end{proof}


{{\lemma{An optimal solution of constrained optimization $P_{\mathcal{C}}$ over constraint $\mathcal{C}$ is always a Pareto optimal solution to the corresponding MOO problem.
\label{prop:constr_optimal}}}
\begin{proof}
	Proof by contradiction.
	
	\bm{$f^*$} is the solution to the constraint optimization problem $P_{\mathcal{C}}$.
	Suppose there exist a \bm{$f'$} that is a solution to the MOO problem and  Pareto dominates \bm{$f^*$}. This implies for some $j$, $f_j' < f_j^*$ and $f_l' \leq f_l^*$ for any $l$ such that $ 1 \leq l \leq k$ and $l \ne j$.
	
	Switch the role of $P_{\mathcal{C}}$ to make $F_j(\bm{x})$ as the objective, call this new constraint optimization problem $P_{\mathcal{C^{''{\tiny }}}}$. By Proposition \ref{prop:dual_optimal}, \bm{$f^*$} is the optimal solution to $P_{\mathcal{C^{''}}}$ .
	
	Construct another constraint optimization problem $P_{\mathcal{C'}}$ using \bm{$f'$} (in place of $\mathcal{C}$) and put $F_j(\bm{x})$ as the objective. It is easy to see \bm{$f'$} is a feasible solution to $P_{\mathcal{C'}}$.
	
	By assumption $f_l' \leq f_l^*$ for any $l$ such that $ 1 \leq l \leq k$ and $l \ne j$, $P_{\mathcal{C^{''}}}$ is a relaxation of $P_{\mathcal{C{'}}}$. \bm{$f'$} is a feasible solution to $P_{\mathcal{C^{'}}}$ implies it is also a feasible solution to $P_{\mathcal{C^{''}}}$, it can not dominate \bm{$f^*$} which is the optimal solution of $P_{\mathcal{C^{''}}}$.	
\end{proof}

The above result shows that solving a CO problem can lead to a Pareto optimal point. We next explain how exactly we construct the CO problem given $k$ objectives. To present our solution, we repeat some definitions used in the NC method~\cite{messac2003nc} below.

\definition{{\bf Reference Point:} \bm{$r_i$} is a special Pareto optimal point if it achieves the minimum for  objective $F_i$.}
\cut{
Since finding \bm{$r_i$} is a single objective optimization problem, it can be solved directly. For a $k$-objective optimization problem, there exist $k$ different reference points.
}
\definition{{\bf Utopia and Nadir Points:} \bm{$r^1$}, $\ldots,$  \bm{$r^k$} $\in \Phi$} are $k$ reference points. A point \bm{$f^U$} $\in \Phi$ is a Utopia  point iff for each $i = 1,2,...,k$, $f^U_i$ $=\min_{l=1}^k \{r^l_i\}$}. A point \bm{$f^N$} $\in \Phi$ is a Nadir point iff for each $i = 1,2,...,k$, $f^N_i$ $=\max_{l=1}^k \{r^l_i\}$}. 
\vspace{0.1in}
%\definition{\bf{Nadir Point:} \bm{$r^1$}, $\ldots,$  \bm{$r^k$} $\in \Phi$} are $k$ reference points. A point \bm{$f^N$} $\in \Phi$ is a Nadir point iff for each $i = 1,2,...,k$, $f^N_i$ $=\max\{r_i\}$}.

The Utopia point and Nadir point indeed are the two extreme points that form a hyperrectangle in the objective space. Every point in this hyperrectangle Pareto dominates the Nadir point and is dominated by the Utopia point. The Pareto frontier can be arbitrary shape within this hyperrectangle without further information.

Next we describe a method to find {\bf one} Pareto point enclosed by the Utopia point and the Nadir Point. 
%which is the Middle point probe. %The definition of uncertain space is postponed to the next section. 
\cut{
For now, one can interpret uncertain space as the hyperrectangle enclosed by the Utopia point and the Nadir Point: a Pareto point can exist anywhere within it.
}
\definition{{\bf Middle Point Probe:}  Given a hyperrectangle formed by \bm{$f^U}$ = $(f_1^U, \ldots, f_i^U, \ldots, f_k^U)$ and  \bm{$f^N$} = $(f_1^N,$ $\ldots, f_i^N, \ldots, f_k^N)$, the middle point \bm{$f^M$} bounded by \bm{$f^U}$ and \bm{$f^N$} is defined as the solution to constrained optimization of:
	\begin{equation}
	\begin{aligned}
	\bm{x}_{\mathcal{C}}=  \hspace{0.2cm} & \underset{\bf\bm{x}}{\text{\bf arg min}}\hspace{0.3cm}F_i(\bm{x}) ,\\
	\text{\bf subject to}\hspace{0.2cm} 
	& F_j(\bm{x}) \leq  \frac{(f_j^U + f_j^N)}{2}, \hspace{0.2cm} j \in [1,k], j \neq i. %m_j =
	\end{aligned}
	\label{eq:opt}
	\end{equation}
}
\vspace{0.05in}

%where $m_j=(f_j^U + f_j^N)/2$.
\noindent{In theory, we can choose any objective to be the objective of the middle point probe.}

\begin{figure}
	\vspace{-0.1in}
	\hspace{-0.2in}
	
	\begin{tabular}{cc}
		\hspace{-0.2in}
		\subfigure[\small{Middle point probe.}]
		%with sublanguages mapped to different complexity classes
		{\label{fig:us_example_2d_1}
			\includegraphics[width=4.2cm]{figures/uncertain_space_2d_1.pdf}}
		
		&
		\hspace{-0.2in}
		\subfigure[\small{multiple Pareto points.}]
		{\label{fig:us_example_2d_2}\includegraphics[width=4.2cm]{figures/uncertain_space_2d_2.pdf}}
		
	\end{tabular}
	\vspace{-0.2in}
	\caption{\small Uncertain space in 2-dimension. \bm{$f^U$} and \bm{$f^N$} are the Utopia and Nadir points, respectively. In (a), \bm{$f^M$}  is the solution to the middle point probe. In (b), (\bm{$f^1$}, \bm{$f^2$}, \bm{$f^3$})  represent the solutions of a series of middle point probes.}
	\label{fig:us_example}
	\vspace{-0.1in}
\end{figure}

In the presence of \bm{$f^M$}, the sub-hyperrectangle enclosed by \bm{$f^M$} and \bm{$f^U$} contains only the points that dominate \bm{$f^M$} (the blue rectangle in Figure \ref{fig:us_example_2d_1}). Due to the Pareto optimality of \bm{$f^M$}, we are certain that no Pareto points exist there. Similarly the sub-hyperrectangle enclosed by \bm{$f^M$} and \bm{$f^N$} (the red rectangle in Figure \ref{fig:us_example_2d_1}) contains only points dominated by \bm{$f^M$}; hence  no Pareto points can exist there. 
%This can be seen in Figure \ref{fig:us_example_2d_1}. 

%Later we will provide the definition of uncertain space. For now, one can interpret it as a set of hyperrectangles where a Pareto point can exist anywhere within it. For example, the red and blue part in Figure \ref{fig:us_example_2d_1} can not be part of the uncertainty space. Hence in finding \bm{$f^M$}, we can reduce the uncertain space by throwing away two sub-hyperrectangles.

{\proposition \label{prop:mid_probe} The middle point probe can reduce the volume of current hyperrectangle by $1 - \frac{1}{2^{k-1}}$ when continuous assumption holds. In the general case, it guarantees to reduce the volume of the current hyperrectangle.}
\begin{proof}
	Denote the volume of a hyper rectangle as $V_{U, N}$ where \bm{$f^U$} and \bm{$f^N$} are the Utopia and Nadir points respectively, \bm{$f^M$} is the middle point calculated by the middle point probe method. By Proposition \ref{prop:equa_constraint}, under the continuous assumption, $f^M_j=(a_j + b_j)/2$ except $j = i$. 
	
	The volume of the original hyper rectangle is: 
	$$V_{U, N}=\prod_{1\leq j \leq k} |f^U_j - f^N_j|$$.
	
	The volume of the sub hyper rectangle enclosed by the Utopia point and Middle point is:
	
	$$V_{U, M}=\prod_{1\leq j \leq k} |f^U_j - f^M_j| = |f^U_i - f^M_i|*\prod_j |\frac{f^U_i - f^N_i}{2}|$$
	
	where $j \in [i,k]$ and $j \neq i$. Similarly 
	
	$$V_{N, M}=\prod_{1\leq j \leq k} |f^N_j - f^M_j| = |f^N_i - f^M_i|*\prod_j |\frac{f^U_i - f^N_i}{2}|$$
	
	Take the sum we have
	$$V_{U, M} + V_{N, M} = \frac{1}{2^{k-1}}\prod_{1\leq i \leq k} |f^M_i - f^N_i| = \frac{1}{2^{k-1}}*V_{U, N}$$
\end{proof}

\minip{A Series of Constrained Optimization Problems.} 
Having explained that a middle point probe defines a CO problem, leading to one Pareto optimal point, 
we next extend our solution  to translate a MOO problem to a series of CO problems in order to cover all (or most) of the Pareto set.

The middle point probe method described above   offers not only a way to find a single Pareto point, but also  a potential iterative method to find more Pareto points. The middle point  \bm{$f^M$} divides the rectangle into $2^k$ sub-hyperrectangles, formed by $k$ hyperplanes that  go through  \bm{$f^M$} and are parallel to the each dimension. %Each is enclosed by two points. 
If we abuse the notation, for each of the sub-hyperrectangles, it is indeed enclosed by its own Utopia point and Nadir point, which can be  easily calculated by \bm{$f^U}$, \bm{$f^N}$, and \bm{$f^M}$. As seen in Figure \ref{fig:us_example_2d_1}, after finding the middle point \bm{$f^M}$, one can form two sub-hyperrectangles,  enclosed by $(U^1, N^1)$ and $(U^2, N^2)$, respectively. 
Based on this observation, we can derive an iterative method to find more Pareto points by recursively invoking the middle point probe for each sub-hyperrectangle formed.

\definition{{\bf Iterative Middle Point Probes:}  
\label{def:iter-probes}
Given the initial Utopia and Nadir points, \bm{$f^U$} and \bm{$f^N$},  in $k$-dimensional objective space, the first middle point probe returns one Pareto point that divides the hyperrectangle enclosed by (\bm{$f^U$}, \bm{$f^N$}) into $2^k$ sub-hyperrectangles. Two of the sub-hyperrectangles can be safely discarded, while others are added to a queue, each of which has its own Utopia and Nadir points, ($U^i$, $N^i$), representing the unexplored space with  no knowledge if Pareto points exist. For each unexplored sub-hyperrectangle, we remove it from the queue and continue to apply the middle point probe: if the probe returns a new Pareto point, we  generate new sub-hyperrectangles and add them to the queue for exploration later. This process continues until the queue is empty or the maximum number of iterations is reached.}
\vspace{0.05in}


%\todo{Fei: Add  results. (1) For 2D problems, we can generate the complete Pareto set. (2) For k>2, we return a subset.  Perhaps add a diagram explaining the differences between 2D and 3D problems? (3) Claim the hardness of this problem and none of the solutions  can guarantee to return all the Pareto points. }

In 2-dimensional space, starting form the Utopia and Nadir points, this method guarantees that in each iteration, it either finds a Pareto optimal point or there is no feasible solution to the corresponding constrained optimization problem. Moreover, in each iteration this method guarantees to reduce the uncertainty space. Further, it guarantees to find all the Pareto points if they are finite. This is because in each iteration, each sub-space is either marked as infeasible for Pareto optimality, or to be explored further in the following iteration. Therefore, it does not  leave any sub-space unexplored or unmarked.
In high-dimensional space, due to the complexity of subspace construction, it is possible that the  method leaves some sub-space unexplored, and hence it can guarantee  to find only a subset of the Pareto optimal points.
\todo{A formal statement?}


\minip{Extension to discrete parameters}. When the continuous assumption of the Pareto frontier is relaxed, in general, it is not guaranteed that the solutions returned are Pareto optimal. This is a fundamental issue when a numerical approach to optimization  has to deal with discrete parameters. However, we can add a filter at the end of our Progressive Frontier approach to remove the solutions that are not Pareto optimal. This is similar to the NC method~\cite{messac2003nc}.



==> related_work_TR.tex <==
\section{Related Work}

\textbf{Parallel Data Stream Systems.} 
%Data stream systems (e.g.,~\cite{Abadi+2005:borealis,ChandrasekaranDFHHKMRRS03,Tatbul+07:shedding})
% laid a foundation for relational  stream processing.
%However, they mainly focused on pipeline parallelism, and hence the degree of parallelism is limited by the depth of the operator graph.
%Techniques for QoS including scheduling and load shedding have been studied in Aurora/Borealis~\cite{Abadi+2005:borealis,Carney03:aurora,Tatbul+07:shedding}. However, scheduling in Aurora~\cite{Carney03:aurora} considers latency only based on CPU costs and selectivity of operators in the single-machine environment, whereas our resource planning considers many more factors in a distributed system and uses constrained optimization to support both latency and throughput. % is based on constraint optimization with a precise cost model that captures unique factors in the more complex distributed architecture such as network.
%Load shedding in Borealis~\cite{Tatbul+07:shedding} allocates resources in a distributed environment by solving a linear optimization problem, but only maximizes throughput without considering latency and only supports pipeline parallelism without data parallelism.
%Earlier distributed stream processing considered
%a distributed federation of participating nodes in different domains~\cite{Abadi+2005:borealis},
%query-aware partitioning of data streams~\cite{Johnson+2008:partitioning},
%and managing analytics artifacts deployed across cloud-edge topologies~\cite{DiAI13}.
Recently there has been a flurry of systems developed for parallel stream processing,  including
Google MillWheel~\cite{Akidau+2013:millwheel}, % Data model~\cite{Google-dataflow2015}, and Percolator~\cite{Peng2010},
Twitter %Storm~\cite{storm} and 
Heron~\cite{Heron2015},
%Facebook Ptail and Puma~\cite{Borthakur:2011},
Microsoft Naiad~\cite{Murray+13:naiad}, 
%Sonora~\cite{Yang+12:sonora},
%and SQL server~\cite{Larson:2015},
SAP Hana~\cite{SAP-realtime},
%WalmartLabs' Muppet~\cite{Lam:2012},
%IBM System S~\cite{Zou+2010:s},
%Yahoo S4~\cite{Neumeyer+2010:s4},
Spark Streaming~\cite{Zaharia+2013:discretized}, and
Flink~\cite{Flink-recovery2015}.
%StreamMapReduce~\cite{Brito+11:streammapreduce},
%StreamCloud~\cite{Gulisano+12:streamcloud},
%SEEP~\cite{CastroFernandez+13:seep} and TimeStream~\cite{Qian+13:timestream}.
%Most of these systems focus on system issues such as fault tolerance, load balancing and elasticity~\cite{Akidau+2013:millwheel,CastroFernandez+13:seep,Flink-recovery2015,Heron2015,Qian+13:timestream,storm,Yang+12:sonora,Zaharia+2013:discretized}.
%Brito+11:streammapreduce,Gulisano+12:streamcloud,
%Some make simplifying assumptions to enable pipeline parallelism, e.g., the complete dataset or a data structure summarizing its related computation fitting in memory~\cite{Murray+13:naiad,Larson:2015,SAP-realtime},
%while others become highly inefficient when the data size exceeds the memory size~\cite{storm,Akidau+2013:millwheel,Zaharia+2013:discretized}.
%The assumption of in-memory processing may hold for %relatively small datasets or
%business analytics  that heavily use aggregation to reduce the data size. It, however, does not hold for broader data analysis. For example, genomic data processing operates on half a terabyte of data per human sample and the data size only grows though the analysis pipeline.
%As a result, despite tremendous effort on system development,
%%the field of big data is left {\bf without  a principled answer} to the above questions,
%the field of big data still lacks an answer to the question of how to support both scale and low latency in a principled approach,
%the industry experiences repeated engineering work,
%and the resulting systems may offer significantly inferior performance to our initial prototype based on
%a principled design~\cite{LiM+11,LiDS15}.
None of these stream systems can automatically address minimizing latency while maximizing throughput. Our proposed work has the potential to benefit all of such systems for performance optimization.

%\textbf{Data Stream Management systems} (e.g.,~\cite{Abadi+2005:borealis,Carney03:aurora,ChandrasekaranDFHHKMRRS03,Shah2004,Tatbul+07:shedding})
% laid a foundation for relational query processing on data streams, including window semantics, incremental algorithms for relational operators, out-of-order data processing, and fault tolerance~\cite{Shah2004}. %and loading balancing
%However, these systems focused on pipeline parallelism, that is, to run a graph of relational operators over pipelined data records called tuples, and hence the degree of parallelism is fundamentally limited by the depth of the graph.
%Techniques for QoS including scheduling and load shedding have been studied in Aurora/Borealis~\cite{Abadi+2005:borealis,Carney03:aurora,Tatbul+07:shedding}. However, scheduling in Aurora~\cite{Carney03:aurora} considers latency only based on CPU costs and selectivity of operators in the single-machine environment, whereas our resource planning considers many more factors in a distributed system and uses constrained optimization to support both latency and throughput. % is based on constraint optimization with a precise cost model that captures unique factors in the more complex distributed architecture such as network.
%Load shedding in Borealis~\cite{Tatbul+07:shedding} allocates resources in a distributed environment by solving a linear optimization problem, but only maximizes throughput without considering latency and only supports pipeline parallelism without data parallelism.


%\textbf{Earlier Distributed Stream Processing.}
%Distributed stream processing has considered
%a distributed federation of participating nodes in different administrative domains~\cite{Abadi+2005:borealis},
%%the routing of tuples between nodes~\cite{Tian+2003:eddies},
%query-aware partitioning of data streams~\cite{Johnson+2008:partitioning},
%and managing analytics artifacts deployed across cloud-edge topologies~\cite{DiAI13}.
%% and  pipelined parallelism for joins \cite{WangR09},
%%without using \mr.
%%These works extend single-node systems to distributed systems, and do not use \mr.
%Our work differs from these techniques as it considers the MapReduce model for cluster computing and extends it to low-latency analytics.
%%\cite{Johnson+2008:partitioning} explores a mechanism for distributed processing of very high speed and volume data streams. The method analyzes given query set and chooses the optimal partitioning scheme. This query-aware data stream method has good scalability.


%\textbf{Parallel stream systems}. The importance of scalable, low-latency analysis has stirred a flurry of system development on parallel stream processing,  including
%Google MillWheel~\cite{Akidau+2013:millwheel,Google-dataflow2015}, % and Percolator~\cite{Peng2010},
%Twitter Storm~\cite{storm} and Heron~\cite{Heron2015},
%%Facebook Ptail and Puma~\cite{Borthakur:2011},
%Microsoft Naiad~\cite{Murray+13:naiad} %Sonora~\cite{Yang+12:sonora},
%and SQL server~\cite{Larson:2015},
%SAP Hana~\cite{SAP-realtime},
%%WalmartLabs' Muppet~\cite{Lam:2012},
%IBM System S~\cite{Zou+2010:s},
%%Yahoo S4~\cite{Neumeyer+2010:s4},
%and
%academic prototypes such as Spark Streaming~\cite{Zaharia+2013:discretized},
%Flink~\cite{Flink-recovery2015},
%%StreamMapReduce~\cite{Brito+11:streammapreduce},
%%StreamCloud~\cite{Gulisano+12:streamcloud},
%SEEP~\cite{CastroFernandez+13:seep} and TimeStream~\cite{Qian+13:timestream}.
%Most of these systems focus on system issues such as fault tolerance, load balancing and elasticity~\cite{Akidau+2013:millwheel,CastroFernandez+13:seep,Flink-recovery2015,Heron2015,Qian+13:timestream,storm,Yang+12:sonora,Zaharia+2013:discretized}.
%%Brito+11:streammapreduce,Gulisano+12:streamcloud,
%Some make simplifying assumptions to enable pipeline parallelism, e.g., the complete dataset or a data structure summarizing its related computation fitting in memory~\cite{Murray+13:naiad,Larson:2015,SAP-realtime},
%while others become highly inefficient when the data size exceeds the memory size~\cite{storm,Akidau+2013:millwheel,Zaharia+2013:discretized}.
%The assumption of in-memory processing may hold for %relatively small datasets or
%business analytics  that heavily use aggregation to reduce the data size. It, however, does not hold for broader data analysis. For example, genomic data processing operates on half a terabyte of data per human sample and the data size only grows though the analysis pipeline.
%As a result, despite tremendous effort on system development,
%%the field of big data is left {\bf without  a principled answer} to the above questions,
%the field of big data still lacks an answer to the question of how to support both scale and low latency in a principled approach,
%the industry experiences repeated engineering work,
%and the resulting systems may offer significantly inferior performance to our initial prototype based on
%a principled design~\cite{LiM+11,LiDS15}.


\textbf{Multi-Objective Optimization}.
General multi-objective optimization approaches includes weighted sum (WS)~\cite{das1997a, marler2004survey}  and normalized constraint (NC)~\cite{messac2003nc}, which we compared in evaluation.
%and evolutionary algorithms~\cite{deb2001multi}. 
WS cannot provide evenly distributed  points on the Pareto frontier, or 
points on non-convex portions of the frontier~\cite{das1997a,messac2012from}. 
Adaptive WS (AWS)~\cite{messac2003nc} can handle non-convex function by recursively calling WS for the segment that does not have any solutions returned, but incurs  much longer running time than WS.
NC aims to provide an evenly distributed Pareto frontier, but its returned solutions are not guaranteed to be Pareto optimal and it is not an incremental algorithm. 
%WS cannot provide evenly distributed  points on the Pareto frontier. 
%It is also known that WS is not able to obtain points on non-convex portions of the Pareto Frontier \todo{in the criterion space}~\cite{das1997a, messac2012from}.
%Adaptive Weighted Sum (AWS) approach, which is a variant of weighted sum approach could handle non-convex function by recursively calling weighted sum approach for the segment which does not have any solutions returned. AWS has much longer running time than WS since WS is invoked many times.
Multi-objective query optimization for SQL queries~\cite{Ganguly:1992:QOP,Kllapi:2011:SOD,Trummer:2014:ASM,TrummerK15, moosigmod2016, moo2sigmod2016} enumerates a finite set of query plans based on relational algebra, and selects the Pareto-optimal ones based on estimated cost of each plan. However, none of them automatically recommend a plan to user. %instead of asking user to choose one manually.
The work~\cite{Kllapi:2011:SOD} addresses workflow scheduling multi-objective optimization, but is a different problem in the parameter space and solution from ours.


\textbf{Resource Management.}
TEMPO~\cite{tan2016tempo} addresses resource management in a database in  the  multi-objective optimization setting. 
%Although cast as a multi-objective optimization (MOO) problem, it actually transforms the MOO problem into a proxy model, which is single-objective optimization and easier to solve. 
When all SLOs cannot be satisfied, it guarantees max-min fairness over SLO satisfactions; otherwise, it degrades to WS for recommending a single solution.
WiseDB~\cite{MarcusP16,MarcusSP17} proposed learning-based techniques for resource management in the cloud.  A decision tree, which is trained on a set of performance and cost-related features collected from minimum cost schedules of sample workloads, is utilized to model the workload characteristics and later for scheduling. In contrast, our deep learning techniques can learn and predict latency and throughput automatically.
Recent  optimization for cluster and cloud computing~\cite{LiNN14,ShiZLCLW14} 
%SmartSLA2015,
still focuses on  running time of relational queries, but not general dataflow problems or multiple objectives.
Dhalion~\cite{Floratou:2017:DSS} uses learning techniques to detect backpressure and resolve it by tuning the degree of parallelism, but does not address the MOO problem.
The work~\cite{Wang:2016:LHO} addresses  cloud pricing  by asking the user to provide statistics and a utility function  and then generating a contract  for the price and completion time. 
OtterTune~\cite{VanAken:2017:ADM} optimizes database queries  by using machine learning to  tune the configuration knobs. However, its workload characteristics are already provided via the DBMS statistics (such as the number of pages read/written, query cache utilization), while our work extracts workload encodings from dataflow programs through deep learning. Moreover, it performs in the space of single objective instead of multi-objectives. 
PerfOrator~\cite{perforator} addresses the problem of finding best hardware resources given an execution plan of SQL queries. PerfOrator supports UDFs but has to keep a sample of the data. It relies on profile runs to update its prediction model that estimates, using non linear regression, the data size at each level of the execution plan. But, to allocate resources, it predicts latency by using hard coded rules that match hardware choice with estimates of the data size at each level.
Recent work in DBMS \cite{kde-vldb, kde-sigmod} tries to optimize query plans by providing better estimates for join and multidimensional selectivities using Kernel Density Estimation (KDE). Kernel density estimation relies on generative models, while the regression models we used are considered to be discriminative models in the machine learning terminology.


%Automatic Database Management System Tuning Through Large-scale Machine Learning [SIGMOD2017]~\cite{VanAken:2017:ADM}
%OtterTune tries to optimize queries run on RDBMS by using machine learning to control and tune the configuration knobs. It mainly differs from our work in: (1) The workload characteristics are provided by leveraging statistics (such as # of pages read/written, query cache utilization) within the RDBMS itself. However, workload extraction constitutes a major contribution and is learned in-situ without prior statistics. (2) Unsupervised learning techniques such as clustering are used in OtterTune to select the most impactful knobs. In our work, we only have 4 parameters to tune, so this is not an issue. (3) OtterTune performs in the space of single objective instead of multi-objectives. The database administrator has to provide the tuning manager with the target to optimize (either latency or throughput).
%Both our work and OtterTune have an approach that maps new workloads to previously seen workloads to leverage their training data.



%\cite{Wang:2016:LHO}
%Lifting the Haze off the Cloud: A Consumer-Centric Market for Database Computation in the Cloud [VLDB2016]
%The paper introduces a system that plays the role of a broker agent between consumer and cloud service providers in order to maximize the user utility regarding completion time of queries and computational cost. The key differences with respect to our work: (1) In our work, we try to do in-situ modeling without using pre-defined analytical models. (2) In this paper, the user has to provide to the broker agent some statistics about the data he uses (histogram, a sample of the data, ...) while our system does not ask the user about any statistics because most of the time, data ingested into streaming systems arrive in real-time (except replay scenarios). (3) The user has to provide the system with a utility function (a function of time and cost he accepts to pay); The broker agent recommends in return a contract that maximizes the expected utility by taking into consideration different completion time probabilities. However, in our work, the system asks the user to give simple constraints on the execution time, computation cost and sustained throughput. canÕt provide statistics about the data since data. Then our system recommends a configuration that best meets the user requirements.

%Dhalion: Self regulating Stream Processing in Heron [VLDB 2017] \cite{Floratou:2017:DSS}
%Dhalion is a framework that provides self-regulation of streaming systems in order to meet some SLOs. Its modular architecture consists of a symptom detection, diagnosis generation and resolution phase. Detecting anomalies relies mainly on unsupervised learning (outlier detection and clustering). This system differs from our work in 4 main points: (1): there are no multi-objective optimization, and the system can only meet 1 SLO at a time (throughput). (2): Diagnosis is done by hard coded analytical rules and does not leverage any machine learning technique. (3): The approach is centered around a backpressure mechanism to detect the maximum sustainable throughput. (we donÕt use any backpressure mechanism in our work) (4): The system controls the degree of parallelism at the knob level (and not a global degree of parallelism parameter), so it determines the degree of parallelism at each stage of the streaming pipeline.


%\cite{kllapi2011schedule} works on a workflow scheduling multi-objective optimization, instead of big and fast data processing system, it is a different problem from our work. In particular, it solves two constraint optimizations which constraint on monetary cost and completion time in respectively. It further proposes an skyline computation algorithm and proposes a metric called dataflow elasticity to measure the tradeoff between monetary cost and completion time. The proposed nested loop optimization approach is specifically designed for data processing flow problem and cannot work for big data system configuration problem in straightforward.
%
%TEMPO~\cite{tan2016tempo} optimizes resource manager configuration in a database. Although it models resource manager configuration as a multi-objective optimization problem, it actually transforms the multi-objective optimization problem into a proxy model, which is actually single optimization and much easier to solve. More specifically, when all SLOs cannot be satisfied, Tempo guarantees max-min fairness over
%SLO satisfactions.
%
%WiSeDB~\cite{MarcusP16,MarcusSP17} offers customized solutions to the workload management problem by recommending cost-effective strategies for executing incoming workloads for a given application. A decision tree, which is trained on a set of performance and cost-related features collected from minimum cost schedules of sample workloads, is utilized to model the workload characteristics. The decision tree model is specifically designed for scheduling, in contrast, the deep learning model proposed in our paper could predict latency and throughput.


%\textbf{SLA in cloud computing}.
%Existing big data systems do not offer an optimization framework, in terms of latency, throughput, and cost, for complex analytics, making it not possible to optimize  data processing to suit different user latency requirements.
%For instance, Service Level Agreement (SLA) in cloud computing focuses on simple object serving and recovery operations (e.g.,~\cite{Dynamo2007}),
%%such as reading and writing objects in a data store
%but not analytical tasks.
%Recent database research on optimization for cluster and cloud computing~\cite{Kllapi:2011:SOD,LiNN14,ShiZLCLW14,SmartSLA2015,Trummer:2014,TrummerK15} still focuses on the total running time of relational queries, but not low latency of individual or important answers.
%%A similar set of limitations can be observed in other domains mentioned above.
%The recent parallel stream system development provides neither guarantee in throughput, latency, or cost, nor an in-depth performance comparison of them because it is unclear which parameters to tune for which performance objective.
%\cut{
%A principled approach to  infrastructure development and performance optimization, as proposed in this research, will bring  a formal framework to  unify the system design for big and fast data, understand its performance, and provide guarantees to the end user.
%}






==> related_work_long.tex <==
\section{Related Work}

\textbf{Data Stream Management systems} (e.g.,~\cite{Abadi+2005:borealis,Carney03:aurora,ChandrasekaranDFHHKMRRS03,Shah2004,Tatbul+07:shedding})
 laid a foundation for relational query processing on data streams, including window semantics, incremental algorithms for relational operators, out-of-order data processing, and fault tolerance~\cite{Shah2004}. %and loading balancing
%These techniques were customized for relational query processing.
%In addition,
However, these systems focused on pipeline parallelism, that is, to run a graph of relational operators over pipelined data records called tuples, and hence the degree of parallelism is fundamentally limited by the depth of the graph.
%Our work leverages state-of-the-art techniques for windowed operations and out of order processing in the new context of the  MapReduce cluster computing.
Techniques for QoS including scheduling and load shedding have been studied in Aurora/Borealis~\cite{Abadi+2005:borealis,Carney03:aurora,Tatbul+07:shedding}. However, scheduling in Aurora~\cite{Carney03:aurora} considers latency only based on CPU costs and selectivity of operators in the single-machine environment, whereas our resource planning considers many more factors in a distributed system and uses constrained optimization to support both latency and throughput. % is based on constraint optimization with a precise cost model that captures unique factors in the more complex distributed architecture such as network.
Load shedding in Borealis~\cite{Tatbul+07:shedding} allocates resources in a distributed environment by solving a linear optimization problem, but only maximizes throughput without considering latency and only supports pipeline parallelism without data parallelism.

\textbf{Earlier Distributed Stream Processing.}
Distributed stream processing has considered
a distributed federation of participating nodes in different administrative domains~\cite{Abadi+2005:borealis},
%the routing of tuples between nodes~\cite{Tian+2003:eddies},
query-aware partitioning of data streams~\cite{Johnson+2008:partitioning},
and managing analytics artifacts deployed across cloud-edge topologies~\cite{DiAI13}.
% and  pipelined parallelism for joins \cite{WangR09},
%without using \mr.
%These works extend single-node systems to distributed systems, and do not use \mr.
Our work differs from these techniques as it considers the MapReduce model for cluster computing and extends it to low-latency analytics.
%\cite{Johnson+2008:partitioning} explores a mechanism for distributed processing of very high speed and volume data streams. The method analyzes given query set and chooses the optimal partitioning scheme. This query-aware data stream method has good scalability.


\textbf{Parallel stream systems}. The importance of scalable, low-latency analysis has stirred a flurry of system development on parallel stream processing,  including
Google MillWheel~\cite{Akidau+2013:millwheel,Google-dataflow2015}, % and Percolator~\cite{Peng2010},
Twitter Storm~\cite{storm} and Heron~\cite{Heron2015},
%Facebook Ptail and Puma~\cite{Borthakur:2011},
Microsoft Naiad~\cite{Murray+13:naiad} %Sonora~\cite{Yang+12:sonora},
and SQL server~\cite{Larson:2015},
SAP Hana~\cite{SAP-realtime},
%WalmartLabs' Muppet~\cite{Lam:2012},
IBM System S~\cite{Zou+2010:s},
%Yahoo S4~\cite{Neumeyer+2010:s4},
and
academic prototypes such as Spark Streaming~\cite{Zaharia+2013:discretized},
Flink~\cite{Flink-recovery2015},
%StreamMapReduce~\cite{Brito+11:streammapreduce},
%StreamCloud~\cite{Gulisano+12:streamcloud},
SEEP~\cite{CastroFernandez+13:seep} and TimeStream~\cite{Qian+13:timestream}.
Most of these systems focus on system issues such as fault tolerance, load balancing and elasticity~\cite{Akidau+2013:millwheel,CastroFernandez+13:seep,Flink-recovery2015,Heron2015,Qian+13:timestream,storm,Yang+12:sonora,Zaharia+2013:discretized}.
%Brito+11:streammapreduce,Gulisano+12:streamcloud,
Some make simplifying assumptions to enable pipeline parallelism, e.g., the complete dataset or a data structure summarizing its related computation fitting in memory~\cite{Murray+13:naiad,Larson:2015,SAP-realtime},
while others become highly inefficient when the data size exceeds the memory size~\cite{storm,Akidau+2013:millwheel,Zaharia+2013:discretized}.
The assumption of in-memory processing may hold for %relatively small datasets or
business analytics  that heavily use aggregation to reduce the data size. It, however, does not hold for broader data analysis. For example, genomic data processing operates on half a terabyte of data per human sample and the data size only grows though the analysis pipeline.
As a result, despite tremendous effort on system development,
%the field of big data is left {\bf without  a principled answer} to the above questions,
the field of big data still lacks an answer to the question of how to support both scale and low latency in a principled approach,
the industry experiences repeated engineering work,
and the resulting systems may offer significantly inferior performance to our initial prototype based on
a principled design~\cite{LiM+11,LiDS15}.

\textbf{SLA in cloud computing}.
Existing big data systems do not offer an optimization framework, in terms of latency, throughput, and cost, for complex analytics, making it not possible to optimize  data processing to suit different user latency requirements.
For instance, Service Level Agreement (SLA) in cloud computing focuses on simple object serving and recovery operations (e.g.,~\cite{Dynamo2007}),
%such as reading and writing objects in a data store
but not analytical tasks.
Recent database research on optimization for cluster and cloud computing~\cite{Kllapi:2011:SOD,LiNN14,ShiZLCLW14,SmartSLA2015,Trummer:2014,TrummerK15} still focuses on the total running time of relational queries, but not low latency of individual or important answers.
%A similar set of limitations can be observed in other domains mentioned above.
The recent parallel stream system development provides neither guarantee in throughput, latency, or cost, nor an in-depth performance comparison of them because it is unclear which parameters to tune for which performance objective.
\cut{
A principled approach to  infrastructure development and performance optimization, as proposed in this research, will bring  a formal framework to  unify the system design for big and fast data, understand its performance, and provide guarantees to the end user.
}

\textbf{Multi-Objective Optimization}.
General multi-objective optimization approaches includes weighted-sum(WS)~\cite{das1997a, marler2004survey}, normalized constraint(NC) method~\cite{messac2003nc}, evolutionary algorithms~\cite{deb2001multi}. 
WS cannot provide evenly distributed  points on the Pareto frontier. 
It is also known that WS is not able to obtain points on non-convex portions of the Pareto Frontier~\cite{das1997a,messac2012from}. 
Adaptive Weighted Sum (AWS) \todo{citation} can handle non-convex function by recursively calling WS for the segment which does not have any solutions returned, but incurs  much longer running time than WS since WS is invoked many times.
NC aims to provide a evenly distributed Pareto frontier, \todo{but cannot guarantee to return the most critical points in case we only want to get a small set of critical points such as knee points.} 
%WS cannot provide evenly distributed  points on the Pareto frontier. 
%It is also known that WS is not able to obtain points on non-convex portions of the Pareto Frontier \todo{in the criterion space}~\cite{das1997a, messac2012from}.
%Adaptive Weighted Sum (AWS) approach, which is a variant of weighted sum approach could handle non-convex function by recursively calling weighted sum approach for the segment which does not have any solutions returned. AWS has much longer running time than WS since WS is invoked many times.


Multi-objective query optimization for SQL queries~\cite{Ganguly:1992:QOP,Kllapi:2011:SOD,Trummer:2014:ASM,TrummerK15} enumerates a discrete set of query plans grounded in relational algebra, and selects the Pareto-optimal ones based on estimated cost of each plan, however, none of them automatically recommends a plan to user, instead of asking user to choose one manually.
The work \cite{kllapi2011schedule} addresses workflow scheduling multi-objective optimization, it is a different problem from our work.
TEMPO~\cite{tan2016tempo} optimizes resource manager configuration.
WiseDB~\cite{MarcusP16,MarcusSP17} proposed learning-based techniques for resource management in the cloud.




